Extending Model-x Framework to Missing Data

One limitation of the most statistical/machine learning-based variable selection approaches is their inability to control the false selections. A recently introduced framework, model-x knockoffs, provides that to a wide range of models but lacks support for datasets with missing values. In this work, we discuss ways of preserving the theoretical guarantees of the model-x framework in the missing data setting. First, we prove that posterior sampled imputation allows reusing existing knockoff samplers in the presence of missing values. Second, we show that sampling knockoffs only for the observed variables and applying univariate imputation also preserves the false selection guarantees. Third, for the special case of latent variable models, we demonstrate how jointly imputing and sampling knockoffs can reduce the computational complexity. We have verified the theoretical findings with two different exploratory variable distributions and investigated how the missing data pattern, amount of correlation, the number of observations, and missing values affected the statistical power.

==> chap1/extended.tex <==
%\begin{definition}[Always observed set]
%	The set $\mathcal{S}$, is always observed if for all missingness patterns $\rb$ with non-zero probability, the observed entries contain the set $\mathcal{S}$, i.e. $o \supseteq \mathcal{S}$.
%\end{definition}
%In other words, missing values should only occur on the non-informative variables.

%Formally, the MB can be defined as follows \cite{xx}:




%We formalize this definitions as below:
%This requires, the missingness mechanisms satisfy the 


%are restricted to a class which 

%A remedy is model-x assumes an accurate generative model $\P_X$ is known and as we will illustrate when the missingness mechanisms are restricted, using this generative model to sample the missing entries is sufficient to preserve the joint distribution between the exploratory variables and the response.

%this generative model can be repurposed for missing data imputation.

%A possible remedy is using the 

%The assumption of model-x
%which states xx.

%can invalidate i) the FDR guarantees by shifting the null hypthosis, ii) shift the underlying generative model to create a mismatch. 

%the assumptions of model-x. 

%In this subsection, we investigate how the accurate generative model assumption of model-x, can enable to 

The intuition from the procedure, if the missing variables only occur on the ``redundant'' features, imputation without the response is an advantage because they remain unimportant. 

On the contrary, model-x assumes there is an accurate generative model, $\P_X$ to begin with. As we will show in this subsection, when the missing values occur in ``redundant'' features, repurposing this generative model for imputation can be sufficient for FDR control. For that reason we begin by defining this informative set.


Our first solution referred to as posterior sampled imputation aims to use keep the imputed vectors distribution intact. That is practically very useful because a knockoff sampler $P_{\Xt \mid X}$ of $P_X$ which is already implemented can be applied directly to the imputed matrix. The following Lemma \ref{lem:mar} illustrates the idea.

We first introduce conditions when the null hypothesis set remains invariant.

% We start by introducing the posterior sampled missing value knockoffs method which allows reusing the existing knockoff samplers under MAR and MCAR. 



Next we discuss how to preserve the geneartive model valid.

To help with proving the proposition, we first introduce and prove the following Lemma which states under the same conditions as Proposition \ref{label:b}, the conditional distribution of the missing variable given the remaining variables takes a simplified form.

\begin{lem}\label{aa}
	Assume MAR condition holds, and there exists an always observed set $\mathcal{M}$ which is a Markov Blanket of the Y. Then, for all missingness pattern, $r$, with non-zero probability, given the observed variables, the variables with missing values are conditionally independent of the response and missingness mechanism taking the pattern $r$,
	\[X_m \indep Y, R=\rb \mid X_o\]
	
	%	Let $\Xh=(\Xh_1,\dots,\Xh_p)^T$ denote the imputed vector where $\Xh_o=X_o$. If $\hat{X}_m\sim P_{X_m\mid X_o,R}(\cdot;X_o,R)$ and then $P_X=P_{\Xh}$.
\end{lem}
\begin{proof}
	Statement given in Lemma \ref{prop:a}, $X_m \indep Y, R=\rb \mid X_o$, can be proved by 
	using contraction property \cite{pearlchap1} and combining two simpler conditional independence statements. The first statement states for all probable $\rb$, the missing variables will be independent of the missingness pattern being $\rb$ given the remaining variables and the response, i.e. 
	\begin{equation}\label{eq:b_proofa}
		X_m \indep R=\rb \mid X_o, Y
	\end{equation}
	This statement follows from the definition of MAR which is assumed in Lemma \ref{prop:a}.
	
	The second statement states for all probable $\rb$, missing variables are conditionally independent of the response given the observed variables i.e.
	\begin{equation}\label{eq:b_proofb}
		X_m \indep Y \mid X_o
	\end{equation}
	To show \eqref{eq:b_proofb} holds, we will start with the definition of MB which states all variables xx,
	\begin{align*}
		&X_{M'} \indep Y \mid X_M
		\intertext{For all probable $\rb$, because MB is an always observed set, it's within the observed entries $o$. Combined with the fact $o$ and $m$ forms a partition, the variables outside of MB can be split as follows:}
		=&X_{m},X_{o\setminus M} \indep Y \mid X_M\\
		\intertext{This equation by the weak union property of \cite{pearlchap1} implies}
		\implies &X_m \indep Y \mid X_M, X_{o\setminus M}
		\intertext{Because M is a subset of $o$, it becomes }
		= &X_m \indep Y \mid X_{o}
		%		\stepcounter{equation}\tag{\theequation}\label{}
	\end{align*}
	
	Now we have shown \eqref{eq:b_proofb} holds. This combined with equation \eqref{eq:b_proofa}, following the contraction property \cite{pearlchap1}, imply the Lemma \ref{prop:a} main statement holds i.e.
	\[\implies  X_m \indep Y, R=\rb \mid X_o\]
\end{proof}
Lemma 1 has an important correlary if it holds the imputation function, does not rely on the response then the null set will be preserved. It can also be unrealistic because if you know the ``redundant ones'' can contain missing data you can simply discard those columns. This second condition holds for example, when 
Formally, the MB can be defined as follows \cite{xx}:

\begin{definition}
	Let $\mathcal{M}\subseteq\{1,\dots,p\}$. $X_{\mathcal{M}}$ is the Markov Blanket of $Y$ if xx
	\[Y\indep X_{\overline{\mathcal{M}}} \mid X_\mathcal{M}\]
	holds.
\end{definition}


Now we proceed to proving Proposition \ref{prop:b}. 

\begin{proof}[Proof of Proposition \ref{prop:b}]
	To show Proposition \ref{prop:b} holds, we refer to \eqref{eq:back} in Section \ref{sec:b_background}, which states the difference between the original joint distribution, $\P_{X,Y}$, and the joint distribution resulting from imputation, $\P_{\Xh,Y}$ equals to the weighted sum of the differences between the imputation model's conditional probability $Q_{X_m\mid X_o}$ and the underlying true conditional distribution of the missing variables given all remaining variables, i.e.
	\begin{align*}
		\P_{\hat{X},Y}(\x,y)&-\P_{X,Y}(\x,y)\\
		&=\sum_{\rb}\P_R(\rb)\P_{X_o,Y\mid R}(\x_o,y\mid  \rb)\left[Q_{X_m\mid X_o}(\x_m\mid  \x_o)-\P_{X_m\mid X_o,Y, R}(\x_m\mid  \x_o,y, \rb)	\right]\\
		\intertext{Here, because MAR condition holds, and the MB of Y is an always observed set, Lemma \ref{prop:a} applies. Accordingly, the true conditional distribution  of the missing variables is independent of the response and the missingness mechanism i.e. $X_m \indep Y, R=\rb \mid X_o$.}
		&=\sum_{\rb}\P_R(\rb)\P_{X_o,Y\mid R}(\x_o,y\mid  \rb)\left[Q_{X_m\mid X_o}(\x_m\mid  \x_o)-\P_{X_m\mid X_o}(\x_m\mid  \x_o)
		\right]\\
		\intertext{Plugging in the assumption of Proposition \ref{prop:b}, which states the imputation model matches the conditional distribution of the missing variables given the observed exploratory variables, i.e. $Q_{X_m\mid X_o}=P_{X_m\mid X_o}$}
		&=\sum_{\rb}\P_R(\rb)\P_{X_o,Y\mid R}(\x_o,y\mid  \rb)\left[\P_{X_m\mid X_o}(\x_m\mid  \x_o,y, \rb)-\P_{X_m\mid X_o}(\x_m\mid  \x_o,y, \rb)\right]\\
		&=0
		\stepcounter{equation}\tag{\theequation}\label{}\\
	\end{align*}
	We showed when the MAR condition holds, the MB of Y is an always observed set, and imputation $Q_{X_m\mid X_o}=P_{X_m\mid X_o}$,
	then, as claimed in Proposition \ref{prop:b}, the resulting joint distribution of the variables and response will be preserved i.e. $P_{X,Y}=P_{\Xh,Y}$
	%, which implies $P_{X,Y}=P_{\Xh,Y}$ holds if the imputation model exactly matching the underlying distribution of the missing values conditioned on the observed exploratory variables, response and the missingness pattern $\P_{X_m\mid X_o,Y, R=\rb}$.
	
	
	%$Q_{X_m\mid X_o}=P_{X_m\mid X_o}=\P_{X_m\mid X_o,Y, R}$ holds.
	
	%\[\sum_{\rb}\P_R(\rb)\P_{X_o,Y\mid R}(\x_o,y\mid  \rb)\left[Q_{X_m\mid X_o}(\x_m\mid  \x_o)-\P_{X_m\mid X_o,Y, R}(\x_m\mid  \x_o,y, \rb)\]
	
\end{proof}
One important implication is xx

\begin{cor}
	Under the assumptions of Propositions \ref{prop:b}, the null hypothesis set under fully observed data is equal to the null hypothesis set after imputation  i.e.  $\mathcal{\hat{H}}_0=\mathcal{H}_0$.
\end{cor}
\begin{proof}
	Proof simply follows from the fact that resulting joint distribution of the variables and response will be preserved i.e. $P_{X,Y}=P_{\Xh,Y}$.
\end{proof}
%\begin{lem}\label{lem:mar}
%	Let $\Xh=(\Xh_1,\dots,\Xh_p)^T$ denote the imputed vector where $\Xh_o=X_o$. If $\hat{X}_m\sim P_{X_m\mid X_o,R}(\cdot;X_o,R)$ and then $P_X=P_{\Xh}$.
%\end{lem}
%The proof simply uses Eq. \ref{eq:back} and replaces $Q$ with $P_{X_m\mid X_o,R}(\cdot;X_o,R)$. It's unrealistic in practise to assume the joint distribution of the exploratory variables and the missing data pattern i.e. $P_{X,R}$ to be known. Therefore, we focus our attention on two missing data configurations namely configurations Missing Completely At Random (MCAR) and Missing At Random (MAR) \citep{littleStatisticalAnalysisMissing2002a}. MCAR holds if $X \indep R$ holds and MAR holds if $X_m \indep R \mid X_o$ holds for any $X_m,X_o$ \cite{littleStatisticalAnalysisMissing2002a,mohanGraphicalModelsInference2017}.
%
%\begin{cor}\label{cor:mar}
%	Under MAR or MNAR, if $\hat{X}_m\sim P_{X_m\mid X_o}(\cdot;X_o)$ then $P_X=P_{\Xh}$.
%\end{cor}
%The proof simply follows directly from the conditional independence assumptions of MAR and MNAR. Corollary \ref{cor:mar} is more realistic as it only requires the distribution $P_X$ which we already assumed to be known. We formalize our idea of posterior sampled imputation and reusing a knockoff sampler in the following step.



% The idea behind the first algorithm is simple, 
% The knockoffs framework assumes that the input distribution $P_X$ is known or known to a certain accuracy. That information can be used for imputation in such a way that the FDR control is maintained. The idea is if we can sample $\hat{X}_m$ from the posterior distribution $P_{X_m\mid X_o}$ than the joint distribution of $\hat{X}$ will remain unchanged. More importantly existing knockoff samplers can be used with the same FDR guarantees. 
\vspace{0.5cm}
\begin{definition} Following \cite{barberRobustInferenceKnockoffs2019} a conditional distribution $P_{\Xt\mid X}$ is pairwise exchangeable with respect to a probability distribution $Q_{X}$ if given
	$X\sim Q_X(\cdot)$ and $\Xt\mid X \sim P_{\Xt\mid X}(\cdot;X)$, $X$ and $\Xt$ are pairwise exchangeable.
	
\end{definition}

\begin{cor}
	Under the assumptions of Propositions \ref{prop:b}, If $\Xt \sim P_{\Xt\mid X}(\cdot;\hat{X})$ and $P_{\Xt\mid X}$ is pairwise exchangeable with respect to $P_X$, then $\hat{X}$ and $\Xt$ are pairwise exchangeable.
\end{cor}
%\begin{thm}\label{thm:main}
%	Let $\Xh=(\Xh_1,\dots,\Xh_p)^T$ denote the imputed vector where $\hat{X}_m\sim P_{X_m\mid X_o}(\cdot;X_o)$ and $\Xh_o=X_o$. We assume the distribution $P_{X,R}$ satisfies MCAR or MAR. If $\Xt \sim P_{\Xt\mid X}(\cdot;\hat{X})$ and $P_{\Xt\mid X}$ is pairwise exchangeable with respect to $P_X$, then $\hat{X}$ and $\Xt$ are pairwise exchangeable.
%\end{thm}

% \paragraph{Proof}
\begin{proof}
	
	Following from Proposition \ref{prop:b},
	resulting joint distribution of the variables and response will be preserved i.e. $P_{X,Y}=P_{\Xh,Y}$ and from xx $P_{X}=P_{\Xh}$ also holds. Then $P_{\Xt\mid X}$ is pairwise exchangeable with respect to $P_{\hat{X}}$ and by the definition of a pairwise exchangeable distribution $\hat{X}$ and $\Xt$ are pairwise exchangeable.
	% $\hat{X}\sim P_{X}$ following Lemma \ref{lem:main1}
	
	% \[(\hat{X},\Xt)_\swap \eqd \hat{X},\Xt\]
	
\end{proof}

==> chap1/miss/main.tex <==

% \input{tex/abstract}

% \input{tex/background2}
% \input{tex/background}

\input{tex/intro_new}
% \input{tex/background}
\input{tex/background_nips}
% \input{tex/def_post}
\input{tex/theory_post2}
\input{tex/theory_uni}
\input{tex/theory_err}
\input{tex/latent_sesia}
% \input{tex/latent_gz_2}
\input{tex/exp}
\input{tex/exp_mvn}
\input{tex/results_mvn_p700}
\input{tex/exp_hmm}
\input{tex/results_hmm}


% % \input{tex/experiments_mvn}
% % \input{tex/results_mvn}
% % \input{tex/results_mvn_p700}
% \input{tex/discussion}


\input{tex/contr}
% \input{tex/ack}

==> chap1/miss/tex/abstract.tex <==
One limitation of the most statistical/machine learning-based variable selection approaches is their inability to control the false selections. A recently introduced framework, model-X knockoffs, provides that to a wide range of models but lacks support for datasets with missing values. In this work, we discuss ways of preserving the theoretical guarantees of the model-X framework in the missing data setting. First, we prove that sampling the missing values from their posterior distribution allows reusing existing knockoff samplers in the presence of missing values. Second, we show that sampling knockoffs only for the observed variables and applying univariate imputation also preserves the false selection guarantees. Third, for the special case of latent variable models, we demonstrate how jointly imputing and sampling knockoffs can reduce the computational complexity. We have verified the theoretical findings with two different exploratory variable distributions and investigated how the amount of correlation, the number of observations, and missing values affected the statistical power.

==> chap1/miss/tex/ack.tex <==
\section*{Acknowledgments}

We would like to thank Dr. Alex Gittens for our valuable discussions.

\section*{Funding}

National Institutes of Health (R01 HL145411)

==> chap1/miss/tex/app_alg.tex <==
\subsection{Univariate Sampled Imputation}
We describe how Theorem \ref{thm:uni} can be applied to N i.i.d. observations in Algorithm \ref{alg:uni}.

\begin{algorithm}[H]
\caption{Univariate sampled missing value knockoffs}\label{alg:uni}
\begin{algorithmic}
\STATE {\bfseries Input:} $\{x^{(i)}_{o^{i}}\}_{i=1}^N, \{m^{i},o^{i}\}_{i=1}^N, \{P_{\Xt_{o^i}\mid X_{o^i}}\}_{i=1}^N, P_X$
 \FOR{\texttt{$i=1,\dots,N$}}
    \STATE $m\leftarrow m^i$
    \STATE $o\leftarrow o^i$
    \STATE $\xt_o \sim P_{\Xt_o\mid X_o}(\cdot;x_o^{(i)}) $\hfill\COMMENT{Knockoff Sampling for $X_o$}
    \FOR {$j= 1,...,|m|$}
        \STATE $\hat{x}_{m_j}\sim P_{X_{m_j}}(\cdot)$\hfill\COMMENT{Uni. Imputation of Originals} 
        \STATE $\xt_{m_j}\sim P_{X_{m_j}}(\cdot)$\hfill\COMMENT{Uni. Imputation of Knockoffs} 
    \ENDFOR
    \STATE $\hat{x}^{(i)}\leftarrow(x_o^{(i)},\hat{x}_m)$
    \STATE $\xt^{(i)}\leftarrow(\xt_o,\xt_m)$
\ENDFOR
 \STATE {\bfseries Output:} $x_c,\xt$ 
\end{algorithmic}
\end{algorithm}

\subsection{HMM Latent Variable Posterior Sampling}

% \section{
Given $x_o$, we define $o(t)\defeq o\cap\{1,\dots,t\}$. Algorithm \ref{alg:hmm_post} is an extension of the ``Forward backward sampling for a HMM'' of \cite{sesiaGeneHuntingHidden2019} to the missing data setting. In the missing data setting, multiplication with the emission probabilities $P_{X_t\mid Z_t}$ needs to be applied only if $t$ is observed. That is equivalent to setting the emission probabilities to one for missing values as discussed in
\cite{broman2009guide} Appendix D.2. We provide the theoretical justification in Prop. \ref{thm:hmm_post} for completeness.

\begin{algorithm}[H]
\caption{HMM Latent Posterior Sampling with Missing Values}\label{alg:hmm_post}
\begin{algorithmic}
\STATE {\bfseries Input:} $x_o, P_{Z_1}, P_{X\mid Z}$,$P_{\Zt \mid Z}, o$
\FOR{\texttt{$t=1,\dots,T$}}
    \IF{ $t=1$}
        \STATE $\alpha_t(z_t) \leftarrow P_{Z_1}(z_1)$
    \ELSE 
        \STATE $\alpha_t(z_t) \leftarrow  \sum_{z_{t-1}}P_{Z_t\mid Z_{t-1}}(z_t; z_{t-1})\alpha_{t-1}(z_{t-1})$
    \ENDIF
    \IF{$t\in o$}
    \STATE $\alpha_t(z_t) \leftarrow \alpha_t(z_t)P_{X_t\mid Z_t}(x_t;z_t)$
    \ENDIF
\ENDFOR
\FOR{\texttt{$t=T,\dots,1$}}
    \IF{$t=T$}
        \STATE $P_{\hat{Z}_T\mid X_{o}}(z_T;x_{o})\leftarrow\dfrac{\alpha_{t}(z_t)}{\sum_{z_t'}\alpha_{t}(z_t')}$
        \STATE $\hat{z}_T\sim P_{\hat{Z}_T\mid X_{o}}(\cdot;x_{o})$
    \ELSE
        \STATE $P_{\hat{Z}_t\mid \hat{Z}_{t+1},X_{o(t)}}(z_t;z_{t+1},x_{o(t)})\leftarrow\dfrac{P_{Z_{t+1}\mid Z_t}(z_{t+1};z_t)\alpha_{t}(z_t)}{\sum_{z_t'}P_{Z_{t+1}\mid Z_t}(z_{t+1};z_t')\alpha_{t}(z_t')}$
        \STATE $\hat{z}_t\sim P_{\hat{Z}_t\mid \hat{Z}_{t+1},X_{o(t)}}(;\hat{z}_{t+1},x_{o(t)})$
    \ENDIF
\ENDFOR
\STATE {\bfseries Output:}  $\{\hat{z_t}\}_{t=1}^T$ 
\end{algorithmic}
\end{algorithm}

==> chap1/miss/tex/app_err.tex <==
\subsection{Proposition \ref{thm:err}}\label{app:err}


\begin{proof}[Proof of Proposition \ref{thm:err}]

The MSE of the univariate sampling $Y'$ is given as 

\begin{subequations}\label{eq:mse_uni}
\begin{align}
        \E[(Y-Y')^2]&=\E[Y^2]+\E[Y'^2]-2\E[Y]\E[Y']\\
        &=2\E[Y^2]-2\E[Y]^2\\
        &=2\var(Y)
\end{align}
\end{subequations}
The first line uses $Y\indep Y'$ and expectation is a linear operator. The second line follows from $Y\eqd Y'$.

The conditional MSE of the posterior sampled estimator $Y''$ is given by:

\begin{subequations}\label{proof:mse1}
\begin{align}
    \E[(Y-Y'')^2\mid X]&=\E[Y^2\mid X]+\E[Y''^2\mid X]-2\E[Y\mid X]\E[Y''\mid X]\\
    &=2\E[Y^2\mid X]-2\E[Y\mid X]^2\\
    &=2\var(Y\mid X)\\
\end{align}
\end{subequations}
The first line uses $Y\indep Y''\mid X$ and expectation is a linear operator. The second line uses $Y\eqd Y''$. Then, the MSE of $Y''$ is given as:
\begin{subequations}
\begin{align}
    \E[(Y-Y'')^2]&=\E[\E[(Y-Y'')^2\mid X]]\\
    &=2\E[\var(Y\mid X)]\\
    &=2(\var(Y)-\var(\E[Y\mid X]))\\
\end{align}
\end{subequations}

The first line uses law of iterated expectations and the last line uses the law of total variance.

From Eq. \ref{eq:mse_uni} and Eq. \ref{proof:mse1} it follows that $\E[(Y-Y'')^2]\leq\E[(Y-Y')^2]$. Because ${Y'''=\E[Y\mid X]}$ is the optimal MSE estimator \cite{bertsekas2008introduction}, it has the lowest MSE i.e. ${\E[(Y-Y''')^2]\leq \E[(Y-Y'')^2]}$. 
\end{proof}

==> chap1/miss/tex/app_hmm.tex <==
\section{HMM Experiments}
\subsection{HMM Simulation Parameters}\label{app:hmm}

We have used the simulation parameters in \cite{sesiaGeneHuntingHidden2019}. Let $Z_t$ denote the t'th hidden states and $X_t$ the t'th explonatory variable both are categorical R.Vs with range \{0,\dots,8\}. The transmission and emission probabilities given as follows: 

\[P_{Z_1}(x)=\begin{cases}
    1,&\text{if } x=1\\
    0,              &\text{otherwise}
\end{cases}\]
\[
P_{Z_t\mid Z_{t-1}}(x;y)=\begin{cases}
    0.9,&\text{if } x=y,\\
    0.1,&\text{if } x=y+1 \\
    0.1,&\text{if } x=0, \ y= 8\\
    0,              &\text{otherwise}
\end{cases}
\]
\[
\]
\[P_{X_t\mid Z_{t}}(x;z)=\begin{cases}
    0.35/2,&\text{if } x=z\\
    0.35/2,&\text{if } x=z+1 \\
    0.35/2,&\text{if } x=0, z=8\\
    0.65/7, &\text{otherwise}
\end{cases}
\]

\subsection{Additional Results}

We included the power and FDR figures for our modified Sesia HMM Knockoffs (Algorithm \ref{alg:sesia}). We have also provided constant power contour plots of both posterior sampling + Sesia HMM and modified Sesia HMM Knockoffs in Fig. \ref{fig:contour}.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.\linewidth]{img/hmm/special_hmm.png}
    % {img/Picture2_fill.png}
    \caption{Heatmap of power on the left, FDR on right. Modified Sesia HMM Knockoffs (Algorithm \ref{alg:sesia}) is used. On the left darker red (blue) indicates higher (lower) power. On the right values above $q=0.1$ are red and below are blue.}
    \label{fig:heatmap2}
\end{figure}

\begin{figure}[!h]
    \centering
    \includegraphics[width=1.\linewidth]{img/hmm/left_impute_contr.png}
    \caption{Contour plots of power. Each cross is a searched pair. Interpolation is used to to draw constant power lines. Left: the posterior imputation + Sesia HMM Knockoffs (Algorithm \ref{alg:main}), Right is the Modified Sesia HMM Knockoffs (Algorithm \ref{alg:sesia})}
    \label{fig:contour}
\end{figure}

==> chap1/miss/tex/app_knockoff_setup.tex <==
\section{}
\section{Knockoffs Setup:}\label{app:knock}
In the model-x knockoffs framework one has to specify the feature-scorer and the final weighted score of each variable. As the feature-scorer we have used the coefficients of an L1 regularized logistic regression of the concatenated matrix $[\Xb,\Xtb]$ which optimizes the following objective function:

\[\hat{\beta}, \hat{\beta}_0 = \argmin_{\beta,\beta_0} \sum_{i=1}^N \log(1+e^{-y_i(\beta^T[x^{(i)},\xt^{(i)}]+\beta_0)})+\lambda \norm{\beta}_{1}\]

In each trial $\lambda$ is selected using 5-fold-cross-validation with area under the curve metric and search space $\{1e-10,1e-2,1e-1,1,1e1\}$ is used. Scikit-learn library \cite{scikit-learn} is used for the implementation. Let $\lambda_{cv}$ denote the resulting parameter and $\hat{\beta}(\lambda_{cv})\in \real^{2p}$ denote the estimated coefficients, the feature scores and the final scores are given by: $i=1,\dots, p$, $T_i=|\hat{\beta}(\lambda_{cv})_i|$ and $\Tt_i=|\hat{\beta}(\lambda_{cv})_{i+p}|$. 

==> chap1/miss/tex/app_mvn.tex <==
\clearpage
\section{MVN Experiments}
\subsection{Results}\label{app:mvn}
\begin{figure*}[!htb]
    \centering
    \includegraphics[width=1.\linewidth]{img/mvn/mode_2.png}
    \caption{Comparison of different imputation methods. Left column is power vs $\rho$ and right column is FDR vs $\rho$. Rows corresponds to different amounts of missing data. From top to bottom $p_0$ takes the values $\{0, 0.1, 0.2, 0.3, 0.4\}$. The corresponding color and line style of the imputation methods are denoted in the legend.}
    \label{app:fig:mvn4}
\end{figure*}

==> chap1/miss/tex/back/experiments_insight.tex <==

% \paragraph{Description}
% Keep $w$ constant, change $N$ and $p_0$, impute the missing values using conditional probability sampling and use missing value compatible knockoffs.
% \begin{itemize}
%     \item Amplitude of the regression coefficients are constant,
%     \item Number of samples and \% missing values varies,
%     \item Missing values only occur at true covariates.
%     \item All the samples are used where missing values are imputed by conditional probabilities and appropriate knockoffs are generated.
% \end{itemize}
\subsubsection{Hypothesis}

\begin{itemize}
    \item FDR control is guaranteed by theory.
    \item As the \% of missing values increases, the power is going to reduce. 
    \item As the number of samples increase, tolerance to missing values increases.
    \item If the power with imputations is larger than the power when the missing values are removed, one can recommend using imputations.
    \item In real world removing the missing values may not be feasible, so imputations can be nessesary. Ex: sufficiently large number of features guarantees at least one missing feature for each row 
\end{itemize}

\subsubsection{Pitfalls}
\begin{itemize}
    
    \item The quality of the imputations increases as the correlation between missing features and remaining features increase. As the correlations among the variables increase identifying the true subset becomes more challenging (power should decrease).

    % \item In genotype studies that use densely measured SNPs exact location of a marker may not be crucial. One can cluster correlated SNPs as in \cite{sesiaGeneHuntingHidden2019} and 
    
\end{itemize}
\subsubsection{Variations of the Experiment}
\begin{itemize}
    \item If missing values are not in $S$, how does imputation effects the performance?
\end{itemize}

==> chap1/miss/tex/background.tex <==
% is useful is a debated topic \cite{}
% An interesting question is under which circumstances impu
\section{Background}

One of the challenges of the model-x framework is sampling knockoffs. If it was possible to sample knockoffs for an arbitrary probability distribution, knockoffs method can be used with any imputation algorithm whose resulting distribution can be derived. However, the lower bounds for the computational complexity of sampling knockoffs indicate the operation is not tractable in general
\cite{batesMetropolizedKnockoffSampling2021}. That suggests while imputing one has to consider the structure of the resulting probability distribution.

Instead of using a separate imputation model, one can treat missing values as hidden variables. Although there are existing algorithms for sampling knockoffs for the hidden variable models they only guarantee the pairwise exchangeability of the observed variables \cite{sesiaGeneHuntingHidden2019,gimenezKnockoffsMassNew2019}. Therefore, even those algorithms essentially impute the hidden variables they do not guarantee the pairwise exchangeability of the imputations.

We have also reviewed how missing values are handled previously in the applications of model-x framework. For example, in \cite{candesPanningGoldModelX2017, masudUtilizingMachineLearning2021} missing values are first imputed and the Multivariate Normal(MVN) distribution is fit to the resulting imputed matrix. Even if the initial distribution is indeed MVN that doesn't guarantee it will remain after the imputation. Another problem can be the dependence among the rows of the resulting imputed matrix as the knockoffs framework assumes independence. In two papers we have observed the complete case analysis is used i.e. the rows with missing values are discarded \cite{jiangKnockoffBoostedTree2021,fuHighdimensionalVariableSelection2021}. Although that doesn't invalidate the guarantees of the knockoffs framework, discarding data can lead to lower statistical power or in certain settings to bias \cite{littleStatisticalAnalysisMissing2002a}.

% In \cite{sesiaMultiresolutionLocalizationCausal2020}, the authors discuss 

% argue that because the imputed missing variants that occur in genome datasets are not informative of for the MB discovery 

% for a specific probability distribution. 

% In general the imputed data is only an approximation and the errors it contains propagates to the later stages of the data-processing pipeline. 


% Different methods have been introduced for sampling pairwise exchangeable random vectors which assumes $P_X$ is known but they do not directly support missing values. In \cite{candesPanningGoldModelX2017} Sequential Conditionally Independent Pairs is introduced which works with arbitrary $P_X$ but not computationally tractable in general. \cite{sesiaGeneHuntingHidden2019} utilized the structure in a Hidden Markov Model and developed a tractable sampling method for it. In the same direction \cite{gimenezKnockoffsMassNew2019} introduced a sampling method for Bayesian networks with latent variables with the restriction that observed variables are conditionally independent given the latent variables. 

% There are also approximate methods for generating samples which don't guarantee the FDR control in general. Second-order knockoffs is one such method \cite{candesPanningGoldModelX2017} which approximates $P_X$ as a multivariate normal and samples a $\Xt$ accordingly. In \cite{romanoDeepKnockoffs2020}, a deep learning architecture namely a moment-matching network is used.

% A recent work \cite{sesiaMultiresolutionLocalizationCausal2020} suggested that imputed variables are not necessarily useful in the context of multivariate conditional independence testing because the imputed variables are conditionally independent given the observed variables. Inspired by that discussion, in this work we explore how the missing values and their imputation affect the conditional independence testing performance in the generalized linear model setting. To do that we first discuss how imputation can be integrated into the knockoffs framework while preserving the FDR guarantees.


==> chap1/miss/tex/background2.tex <==
% Why do we need feature selection
% Objective of feature selection
Feature selection and 

Data-driven methods analyze the relationship between a set of measurements referred to as variables or features. Traditionally, the number of variables measured was limited by challenges in gathering, storing, and processing the data. As the computing technology advanced, the number of variables studied increased as well. Increased number of variables introduced additional problems such as the curse of dimensionality (the number of observations per volume of the measurement space gets lower) and overfitting in the case of multivariate models \cite{liFeatureSelectionData2018}.
Moreover, not all variables are related to the problem studied and can contain measurement errors \cite{chandrashekarSurveyFeatureSelection2014}. Decreasing interpretability of multivariate models with increasing dimensions is also another part of the story \cite{liFeatureSelectionData2018}.

One natural solution is selecting a subset of the features. It's clear how feature selection can be useful but its objective is not as clear cut. For example: according to \cite{kohaviWrappersFeatureSubset1997}, the goal of feature selection is among all possible subsets identifying the one with the highest accuracy for a given algorithm. While in the data-mining context easier to work with models, cleaner datasets, and higher performance are included as the goals of feature selection \cite{liFeatureSelectionData2018}. To address that ambiguity, \cite{tsamardinosPrincipledFeatureSelection2003} defines the objective of feature selection in the supervised setting as identifying the Markov blanket of the target variable. Put into words it means selecting the minimal subset of features which when conditioned on, makes the remaining features statistically independent of the target. 

% The Markov blanket discovery problem also has applications in structure learning of probabilistic graphical models and causal inference \cite{aliferisLocalCausalMarkov2010}.

When selected features are treated as scientific discoveries another important aspect of the problem is to control the false selections. For example, in gene association studies, the subset selected among hundreds-of-thousands of genetic markers are studied further for biological relevance. Limiting the false selections limits the selections resulting from pure chance and can lead to more replicable findings. One approach would be using statistical tests whose null hypothesis corresponds to a variable not being included in the MB. That approach becomes challenging even in the parametric setting with a generalized linear model when the number of features exceeds the number of samples \cite{candesPanningGoldModelX2017}. Therefore, in practise it's not uncommon to observe univariate statistical tests used to select features \cite{trynkaDenseGenotypingIdentifies2011, burtonGenomewideAssociationStudy2007}. Those tests has the null hypothesis of marginal independence with a response variable which is a much looser condition than being outside the MB. Permutation testing can be applied to penalized regression models such as in \cite{arbet} or to random forest \cite{coleman} which lack p-values but can be computationally expensive or use looser null hypothesis.

A recent approach, Model-x knockoffs \cite{candesPanningGoldModelX2017} provides a framework for controlling the expected fraction of false selection even with feature scorers that lack p-values. Knockoffs' flexibility comes from being agnostic to the target conditional distribution ($P_{Y\mid X}$) but it as a trade-off requires accurate knowledge of the input distribution ($P_X$). A false selection in the knockoffs setting corresponds to a feature $X_i$ that is statistically independent of the target $Y$ given the remaining features $X_{-i}$ i.e. $Y\indep X_i\mid X_{-i}$. Although, in general this definition is not equivalent to a variable not belonging to the MB it's a more strict condition than marginal independence. One distinctive trait of the knockoffs framework is for each feature a corresponding synthetic feature, a ``knockoff'', is sampled. To control the fraction of false selections, first the feature scorer (such as a penalized regression model) is applied to an augmented dataset that contains this additional synthetic features. Next, scores are assigned to both the original and synthetic features. Those two steps are done in a special way s.t a score-threshold which provides the desired level of false selection control can be identified by contrasting the scores of the originals and their knockoffs.

Another fundamental problem in data analysis is the problem of missing measurements. In 
missing data can interfere with assumptions in feature selection process and therefore addressing two problems independently might not cut it. The simplest solution would be using only the complete data. Alternatives in the statistical literature can be categorized into three groups: single imputation, multiple imputation, and ``Likelihood-Based Inference with Incomplete Data''(LBID) \cite{littleStatisticalAnalysisMissing2002a} based methods. The challenge would be to maintain the statistical properties of the analyses done without any missing data.


% Most statistical or Machine Learning models by default do not support handling data with missing observations. The simplest solution would be using only the complete data. Alternatives in the statistical literature can be categorized into three groups: single imputation, multiple imputation, and ``Likelihood-Based Inference with Incomplete Data''(LBID) \cite{littleStatisticalAnalysisMissing2002a} based methods. The challenge would be to maintain the statistical properties of the analyses done without any missing data.

The problems selecting a subset of variables and handling the missing data in a principled way are intertwined in practice when missing data is observed in high-dimensional settings. In this work, accepting the objective of feature selection as Markov Blanket discovery, we're interested in understanding how missing data can be used for Markov Blanket discovery.




% than assigns a score to both the originals and synthetic features. The weight assignments and the synthetic feature sampling are done in such a way that if a feature is not informative of the target (given the remaining features), then an original feature on average will have equal weight with its knockoff.

% we will show that in certain cases it's.

% That condition is less strict than the MB but as we will show under certain assumptions those two are equivalent.

% in general is less strict then a variable not belonging to the MB but as we will discuss under


missing data 
% fill that gap by providing false selection control to a wide-range of feature scorers. 

% Model-x knockoffs \textcite{candesPanningGoldModelX2017}, provides a expand false selection control to 

% Model-x knockoffs \textcite{candesPanningGoldModelX2017}, introduces a framework to do false selection control

% alleviates the lack of coverage of statistical hypothesis testing in modern features selections methods.
% such as penalized regression or ML based methods.

% Not to mention the lack of p-values of popular feature selection methods such as penalized regression models or random forests. 

% is challenging as coming up with a statistical test with the null hyptohesis  
% aspect scientific discovery control false

% Model-x Knockoffs framework \cite{candesPanningGoldModelX2017} is originally introduced for providing false selections control to a wide-range of feature selection algorithms. 

The knockoffs method provides a framework for using a wide range of feature selection methods while controlling the false selections. Here, we start by introducing the main theorem behind the knockoffs procedure. Given $X$, a p dimensional random vector, and $Y$, a random variable, the objective of feature selection is described as identifying the Markov blanket of the target $Y$ \cite{candesPanningGoldModelX2017}. Markov boundary of the target is defined as the minimal set of random variables $X_{S^*}$ which satisfy:
\[Y\indep X_{-{S^*}} \mid X_{S^*}\]

% In feature selection, the objective is 

where $X_{-{S^*}}$ denote the remaining random variables. 
% Although ideally one is interested in selecting only the variables in $S$, in practise 
Ideally one is interested in selecting only the true variables but a more obtainable goal can be selecting the true variables as much as possible while limiting the selection of the nulls. That problem can be written as follows:

\[\hat{S} = \argmax_{S} \quad \E\bigm[\mid S\cap {S^*}\mid \bigm] \quad \text{s.t} \quad
\normalfont \E\bigm[\dfrac{\bigm|S\ \cap \ -{S^*}\bigm|}{\text{max}(1,\bigm|S\bigm|)}\bigm]\leq q\]

where $\hat{S}$ denotes the selected subset and the inequality constraint corresponds to the expected fraction of selections that do not belong to the Markov blanket of $Y$. That is also the False Discovery Rate (FDR) \cite{benjaminiControlFalseDiscovery2001} for this problem.

One approach can be computing a test-statistic for each feature such that the i'th variable has the null hypothesis $Y\indep X_i \mid X_{-i}$ and applying BH correction \cite{benjaminiControlFalseDiscovery2001} for controlling the FDR as in \cite{barberControllingFalseDiscovery2015a}. That null hypothesis is equivalent to saying $X_i$ is not KJ-Strongly relevant\footnote{$X_i$ is KJ-Strongly relevant to $Y$ iff $Y\nindep X_i \mid X_{-i}$} to $Y$ \cite{tsamardinosPrincipledFeatureSelection2003} and if there exists a directed probabilistic graphical model which is faithful to the $P_{X,Y}$ then not KJ-Strongly relevant implies not in the Markov Blanket \cite{tsamardinosPrincipledFeatureSelection2003}. In that setting, the described BH correction procedure will also control the expected fraction of selections that are not in the Markov Blanket of the target.

% applying BH correction to those null hyptoh approach described above controls the same FDR. 
% because it can be shown that if $Y\indep X_i \mid X_{-i}$ then $i\in -{S^*}$ \footnote{check}. 

The challenge of course is coming up with those test statistics. As it's common in practice to use univariate tests instead with the null hypothesis $Y\indep X_i$ but that doesn't guarantee $Y\indep X_i \mid X_{-i}$. In general, the test-statistics either require assumptions about the conditional distribution of the target $P_{Y\mid X}$ or use a permutation-based approach. The test statistics might not be valid even if the assumptions of the target distribution holds as in the case of generalized linear models when the number of features exceeds the number of samples \cite{candesPanningGoldModelX2017}. The permutation tests on the other hand can be computationally demanding. 

On the other hand, model-X knockoffs methodology \cite{candesPanningGoldModelX2017} allows controlling the FDR in the context of variable selection while being agnostic to the target conditional distribution $P_{Y\mid X}$. The freedom of the target distribution comes at the price of accurate knowledge of the input distribution $P_X$. 

We assume N i.i.d. samples of p-dimensional random vector $X$ and random variable $Y$ are available and they are denoted by $\{X^{(i)}\}_{i=1}^N$ and $\{y^{(i)}\}_{i=1}^N$. Furthermore, $\Xt^{(i)}$ denotes an additional p-dimensional random vector s.t.  $(X^{(1)},\Xt^{(1)},Y^{(1)}),\dots,(X^{(N)},\Xt^{(N)},Y^{(N)})$ are independent. We use $\Xb$ and $\Xtb$ to refer to the matrices whose rows correspond to different $X^{(i)}$ and $\Xt^{(i)}$ respectively. Similarly, $\Yb$ denotes the vector with elements $y^{(i)}$. 

In knockoffs methodology, given an input data matrix $\Xb$ an additional matrix $\Xtb$ is sampled. That additional matrix is referred to as knockoffs and contains no additional information of the observations of the target $\Yb$. Using both matrices and for each of the features a score $w_i([\Xb,\Xtb],\Yb)$ is estimated where a positive score provides supports for its selection. Finally, a knockoff filter is used to estimate a cut-off based on the distribution of the scores, and features with scores above the cut-off are selected. For the process to enjoy the FDR guarantees, the samples $\Xtb$ and estimated $w_i([\Xb,\Xtb],\Yb)$ scores have to satisfy certain conditions which are described in the following theorem.


\begin{thm}%\label{thm:gz}

Theorem 3.5 of Candes et al. \cite{candesPanningGoldModelX2017}. 

% Let $\Xb\in \real^{N\times p}$ denote the input matrix, $\Yb$ denote the observations of the target, and $\Xtb\in\real^{N\times p}$ denote the knockoffs matrix.



Let $W_i\defeq w_i([\Xb,\Xtb],\Yb)$ denote the score of the i'th feature. Knockoffs+ cut-off at level $q$ is given as follows:
% (which we refer as knockoffs) 

\[\normalfont \tau \defeq \text{min}\bigm\{t>0:\dfrac{1+\bigm|\{j:W_i\leq -t\}\bigm|}{\bigm|\{j:W_i\geq t\}\bigm|}\leq q\bigm\}\]

% Let $\tau$ denote the threshold resulting from knockoffs plus filter at level $q$. 

and $\hat{S}\defeq\{i:W_i\geq \tau \}$. Given $\mathcal{H}_0=\{i:Y\indep X_i \mid X_{-i}\}$ if $\ \forall \ S \subseteq \mathcal{H}_0 $
\[(\Xb,\Xtb)_\swap\eqd \Xb,\Xtb\]
\[w_i([\Xb,\Xtb]_\swap,\Yb)=\begin{cases}
    -w_i([\Xb,\Xtb],\Yb),&\text{if } i\in S\\
    w_i([\Xb,\Xtb],\Yb)&\text{o.w.}
\end{cases}
\]

holds and $\Xtb \indep \Yb \mid \Xb $, then the FDR is controlled at level $q$. Formally:
\[\normalfont \E\bigm[\dfrac{\bigm|\hat{S}\ \cap \ \mathcal{H}_0\bigm|}{\text{max}(1,\bigm|\hat{S}\bigm|)}\bigm]\leq q \]

\end{thm}

Here $\eqd$ denotes the equality in distribution and $\swap$ operator given two input vectors swaps the elements indexed by $S$ in the first vector with the ones in the second and vice versa. The definition for input vectors is defined below and can be applied to matrices (in that case columns are swapped).

Let $\swap:(\real^{p},\real^{p})\rightarrow(\real^{p},\real^{p})$ and $(x,\xt)_\swap = (y,z)$ where 
\[y_i= 
\begin{cases}
    \xt_i,& i\in S\\
    x_i,              &i\notin S
\end{cases}
\quad z_i= 
\begin{cases}
    x_i,& i\in S\\
    \xt_i,              &i\notin S
\end{cases}
\]

As $\mathcal{H}_0$ is not known a-priori, to guarantee the above conditions holds, in general we need to sample $\Xtb$ and select the scoring functions $w_i(\cdot)$ s.t the above conditions holds for all $S\subseteq\{1,\dots,p\}$.

If the first condition $(\Xb,\Xtb)_\swap\eqd \Xb,\Xtb$ holds for all $S\subseteq\{1,\dots,p\}$, then $\Xb,\Xtb$ are said to be pairwise exchangeable. Furthermore, it's easy to see that if $X^{(i)}$ and $\Xt^{(i)}$ are pairwise exchangeable than so does $\Xb,\Xtb$ \cite{candesPanningGoldModelX2017}.

That definition opens up the question of how to sample a pairwise exchangeable random vector. In the original paper, Sequential Conditionally Independent Pairs (SCIP) algorithm is introduced which in theory can sample pairwise exchangeable random vectors for any input distribution $P_X$ \cite{candesPanningGoldModelX2017}. However, the algorithm is not guaranteed to be computationally tractable in general. 

The second condition 
\[w_i([\Xb,\Xtb]_\swap,\Yb)=\begin{cases}
    -w_i([\Xb,\Xtb],\Yb),&\text{if } i\in S\\
    w_i([\Xb,\Xtb],\Yb)&\text{o.w.}
\end{cases}
\]
is easier to satisfy. It's stated in \cite{candesPanningGoldModelX2017} that any $w_i(\cdot)$ can be written in two stages: first estimating scores for both the original and the knockoffs i.e.

\[T,\Tt = (T_1,\dots,T_p),(\Tt_1,\dots,\Tt_p)=t([\Xb,\Xtb],y)\]

s.t. $\forall \ S\subseteq \{1,\dots,p\}$ \[t([\Xb,\Xtb]_\swap,y)=(T,\Tt)_\swap\]

and second using an anti-symmetric function $f_i(x,y)=-f_i(y,x)$ to obtain final scores $W_i=f_i(T_i,\Tt_i)$. Using this formulation one can easily use an existing feature scoring method as $t(\cdot)$ (as long as it satisfies the swap condition) and use a simple anti-symmetric function such as $f_i(x,y)=x-y$ as accompany.


% The first condition 


% The $w_i([\Xb,\Xtb],\Yb)$ has to be 

% is sampled referred to as knockoffs 

% later used to obtain  Finally a knockoff filter is used to obtain a cut-off that controls the FDR and features with scores above the cut-off are selected.


% In knockoffs methodology given a data matrix $\Xb\in \real^{N\times p}$ a knockoff matrix $\Xtb\in\real^{N\times p}$ is sampled which satisfies two conditions: Pairwise exchangibility with $\Xb$ (defined below) and conditional independence with target observations $\Yb\in \real^{N}$ i.e. $\Xtb \indep \Yb \mid \Xb $. The next step is estimating a score for each feature $w_i([\Xb,\Xtb],\Yb)$ using both matrices i

% and the final step is selecting the scores above a cut-off resulting from the knockoff filter.

% \paragraph{Definition}
% Two random vectors $X$ and $\Xt$ are pairwise exchangeable if
% $\forall \ S\subseteq\{1,\dots,p\}$,

% \[(X,\Xt)_\swap \eqd X,\Xt\]



% be pairwise exchangeable with the original matrix and also be independent of the target given 

% , 

% Because a knockoff matrix $\Xtb$ is sampled which

% The freedom in the conditional distribution follows from the assumptions about the input distribution $P_X$.

% which will be used to sample valid knockoffs. 

% That flexibility allows interoperating a wide-range of methods such as generalized linear models (in high dimensional settings), random forests or Bayesian regression \cite{candesPanningGoldModelX2017}. 


% Because the methodology requires valid knockoffs to be sampled which generally requires the knowledge of $P_X$.

% for example allows using ,  such as random forests or other statistical methods such as Bayesian regression \cite{candesPanningGoldModelX2017}. The flexibility of the target conditional distribution $P_{Y\mid X}$ follows from the strict assumptions about the distribution of the input features $P_X$.



% Model-x knockoffs framework \cite{candesPanningGoldModelX2017} allows controlling the False Discovery Rate in the context of variable selection without making assumptions about the target distribution. It requires valid knockoffs to be sampled which generally requires the distribution of $X$. It also can work with a machine learning algorithms such as random forests or other statistical methods such as Bayesian regression under mild assumptions \cite{candesPanningGoldModelX2017}.

% is in a way agnostic to the conditional distribution $P_{Y\mid X}$ and supports a wide-variety of feature selection methods while still maintaining the FDR control in the context of Markov boundary identification.


% There cabe there are methods especially in machine learning used for feature selection neither makes assumptions about the conditional distribution nor provides p-values. 




% as in the case of a linear regression, additional requirements for the sample size might be required. 

% if we assume $P_{Y\mid X}$ follows a generalized linear model, then if the coefficient of the i'th feature is 0 i.e. $\beta_i=0$, then $Y\indep X_i \mid X_{-i}$ holds \cite{candesPanningGoldModelX2017}. The challenge 



% As one either has to make assumptions about $\cite{}$


% Given a matrix $\Xb \in \real^{N,p}$


% With this objective in mind the authors define the null hypothesis for selecting $X_i$ as:
% \[H_0:Y\indep X_i \mid X_{-i}\]

% In traditional feature selection given a data matrix $\Xb$ and target vector $Y$ a subset of features $\hat{S}$ is selected generally by first estimating scores for each feature and then filtering them. 
% In score based feature selection 

% In score based variable selection, a score is attributed to each feature that measures it's relevance to the target. Then, filtering those scores a subset is selected.

% Ideally one is interested in eliminating all the unrelated features. However, generally one faces a trade-off between the number unrelated features and the number of relavent features among the selectionsselected.

% one can be interested in a particular 

% There is a trade-off between the amount of relevant features selected and amount of unrelated 

% If that is not possible a 
% might be desired 

% Modeling and estimation of $Y\mid X$ leads one to make guesses about the conditional 

% Generally, we do not have any labels not given 


% FDR is defined as 
% \[\normalfont \E\bigm[\dfrac{\bigm|\hat{S}\ \cap \ \mathcal{H}_0\bigm|}{\text{max}(1,\bigm|\hat{S}\bigm|)}\bigm]\]




% which obeys the flip-sign condition is selected 




% \is a general framework that works with arbitrary distributions. However, it's not tractable for 



% and has been previously shown to  

% Under which conditions using imputed variables one can recover 
% It's an interesting question under which 





==> chap1/miss/tex/background_nips.tex <==
\section{Background}

In knockoffs methodology, given an input data matrix $\Xb\in\real^{N\times p}$ an additional matrix (called knockoffs) $\Xtb\in\real^{N\times p}$ is sampled such the two matrices are pairwise exchangeable i.e.

\[(\Xb,\Xtb)_\swap\eqd \Xb,\Xtb\]

holds for all $S\in\{1,\dots,p\}$ \citep{candesPanningGoldModelX2017}. The symbol $\eqd$ denotes the equality in distribution and $\swap$ operator given two matrices swaps the columns indexed by $S$ in the first matrix with the ones in the second and vice versa. For that condition to hold, assuming rows of $\Xb$ are i.i.d, each row of $\Xtb$ is sampled using a knockoff sampler i.e. $\Xt^{(i)} \sim P_{\Xt\mid X}(\cdot;X^{(i)})$ s.t. $\Xt^{(i)}$ and $X^{(i)}$ are pairwise exchangeable. In the next step the concatenated matrix $[\Xb,\Xtb]$ and the response $\Yb$, is given to a statistical learning algorithm that assigns weights to each of $2p$ columns i.e.

\[T,\Tt = (T_1,\dots,T_p),(\Tt_1,\dots,\Tt_p)=t([\Xb,\Xtb],y)\]

The only constraint for the statistical learning algorithm is whenever a pair of columns are swapped, the output weights should also be swapped accordingly i.e.  $t([\Xb,\Xtb]_\swap,y)=(T,\Tt)_\swap$  \citep{candesPanningGoldModelX2017}. Next, a knockoffs filter is applied to determine a calibrated threshold $\tau$ as follows \citep{candesPanningGoldModelX2017}:
% (which we refer as knockoffs) 

\[\normalfont \tau \defeq \text{min}\bigm\{t>0:\dfrac{1+\bigm|\{j:T_j-\Tt_j\leq -t\}\bigm|}{\bigm|\{j:T_j-\Tt_j\geq t\}\bigm|}\leq q\bigm\}\]

Finally, the set of features whose original weights are sufficiently higher then its knockoff are selected i.e. $\hat{S}=\{j:T_j-\Tt_j>\tau\}$. If the \pe of $\Xb$ and $\Xtb$ is satisfied, rows of the $[\Xb, \Xtb]$ are independent and the statistical learning algorithm $t(\cdot)$ satisfies the swap condition, then the FDR is controlled at a pre-selected level $q$ as denoted in Eq. \ref{eq:fdr} \citep{candesPanningGoldModelX2017}.

% $\mathcal{H}_0$
Keeping aside the swap condition for the statistical learning algorithm, the \pe condition and the row independence condition has to be justified in practice. To illustrate the effect of missing values imputation on those two assumptions we define the missing data problem next. Let $R=(R_1,\dots,R_p)^T$ denote the missing value indicator R.Vs. $R_j$ takes values in $\{0,1\}$ and $R_j=1$ denotes $X_j$ is missing. Let $m=\{j:R_j=1\}$ and $o=\{1,\dots,p\}\setminus m$ denote the sets of missing and observed values. Given a set $S\subseteq\{1,\dots,p\}$, $X_S=\{X_j:j\in S\}$ denotes the R.Vs indexed by set S. We denote the N i.i.d. observations and masks as $\{X^{(i)}_{o^{i}},R^{(i)}\}_{i=1}^N$ with varying missing values indices $\{m^{i},o^{i}\}_{i=1}^N$.

To understand the effect of imputation on the knockoffs framework, we classified imputation algorithms into two. In the first category, all observed samples are used to impute all missing values jointly as follows:

\[(\hat{X}_{m^1}^{(1)},\dots, \hat{X}_{m^N}^{(N)}) = g(X_{o^1}^{(1)},\dots,X_{o^N}^{(N)})\]

 Matrix completion algorithms \cite{mazumderSpectralRegularizationAlgorithms2010}, and the popular imputation method MICE \cite{van1999flexible}, falls into this category. We denote the $\Xh^{(i)}$ as the resulting imputed random vector where $\Xh^{(i)}_{o^i}=X^{(i)}_{o^i}$ and $\hat{\Xb}$ the resulting $N$ by $p$ imputed matrix. When the knockoffs framework is applied to this new matrix $\hat{\Xb}$ the second assumption of the model-x knockoffs will be violated because of the dependence of the rows. In the second category, missing values are imputed using only the corresponding observed variables \footnote{Dirac delta function can be used to represent deterministic imputation.} i.e. \[\hat{X}_{m}^{(i)}\sim Q_{\Xh_m\mid \Xh_o^{(i)}}(\cdot;X_o^{(i)})\] 
 
 This implicitly assumes the imputation function is assumed to be known apriori (or estimated from a different dataset). But the problem is for an arbitrary $Q_{\Xh_m\mid X_o}$ the resulting distribution of the imputed vector $P_{\Xh^{(i)}}$ is no longer equal to the original $P_{X^{(i)}}$. Dropping the superscripts for brevity, we illustrate this in the Eq. \ref{eq:back}.
 
%   &=\sum_{r}P_{\Xh,R}(x,r)-P_{X,R}(x,r)\\
\begin{subequations}\label{eq:back}
\begin{align}
% \begin{equation}
% \begin{split}
    &P_{\hat{X},Y}(x,y)-P_{X,Y}(x,y)=\sum_{r}P_R(r)\left[P_{\Xh,Y\mid R}(x,y\mid r)-P_{X,Y\mid R}(x,y\mid r)\right]\\
    %
    &=\sum_{r}P_R(r)P_{X_o,Y\mid R}(x_o,y\mid  r)\left[P_{\Xh_m\mid \Xh_o,Y,R}(x_m\mid  x_o,y,r)-P_{X_m\mid X_o,Y,R}(x_m\mid  x_o,y,r)\right]\\
    %
    &=\sum_{r}P_R(r)P_{X_o,Y\mid R}(x_o,y\mid  r)\left[Q_{\Xh_m\mid \Xh_o}(x_m\mid  x_o)-P_{X_m\mid X_o,Y, R}(x_m\mid  x_o,y, r)\right]
\end{align}
\end{subequations}

Briefly \ref{eq:back}a uses the law of total probability and the definition conditional probability. \ref{eq:back}b again uses the definition of conditional probability. In \ref{eq:back}c we use $\Xh_o=X_o$ and the fact that the missing values are imputed using the sampler $Q_{\Xh_m\mid \Xh_o}$. Equation \ref{eq:back} suggests that for an arbitrary 
$Q_{\Xh_m\mid \Xh_o}$ the imputed  distribution is not equal to the original i.e. $P_{\Xh}\neq P_X$.

% Instead of using a separate imputation model, one can treat missing values as hidden variables. Although there are existing algorithms for sampling knockoffs for the hidden variable models they only guarantee the pairwise exchangeability of the observed variables \cite{sesiaGeneHuntingHidden2019,gimenezKnockoffsMassNew2019}. Therefore, even those algorithms essentially impute the hidden variables they do not guarantee the pairwise exchangeability of the imputations.

In our review of the literature, we haven't observed a work that discusses the nuances of missing data in the model-x framework. Missing data is instead either directly imputed or removed for complete case analysis without justification. For example, in \citep{candesPanningGoldModelX2017, masudUtilizingMachineLearning2021} missing values are first imputed and the Multivariate Normal(MVN) distribution is fit to the resulting imputed matrix. This is problematic because first imputed matrix may no longer MVN and next because $P_X$ is estimated from the same data used for feature selection the rows of $\Xtb$ will be dependent. In two papers we have observed the complete case analysis is used i.e. the rows with missing values are discarded \citep{jiangKnockoffBoostedTree2021,fuHighdimensionalVariableSelection2021}. Although that doesn't invalidate the guarantees of the knockoffs framework, discarding data can lead to lower statistical power or in certain settings to bias \citep{littleStatisticalAnalysisMissing2002a}. 

% Despite the obvious effect of imputation, the previous work in model-x literature doesn't  literature model-x

==> chap1/miss/tex/body.tex <==
 % \section{Objective}

% Generating knockoff samples $$

\section{Assumptions}

Let $Z, X$ be two random vectors and $z\in \real^L, x \in \real^p$ respective realizations.
\begin{equation}
    \begin{split}
        z \sim P_Z()\\
        x \sim P_{X\mid Z}(;z)
    \end{split}
\end{equation}

We assume the following conditional independence assumption holds
\[P_{X\mid Z}(x;z)=\prod_{i}P_{X_i\mid Z}(x_i;z)\]

Let us define sets $o\subseteq\{1,\dots,p\}$ and $m=\{1,\dots,p\}\setminus o$ which represent the indices of the observed and missing R.Vs respectively.

The proposed algorithm gives the output $x_m, \xt_o, \xt_m$ given $x_o$ using the following steps:

\begin{equation}
    \begin{split}
        \hat{z} \sim P_{Z\mid X}(;x)\\
        x_m \sim P_{X_m\mid Z}(;\hat{z})\\
        \xt_m \sim P_{X_m\mid Z}(;\hat{z})\\
        \xt_o \sim P_{X_o\mid Z}(;\hat{z})
    \end{split}
\end{equation}

\subsection{Lemma 1}
Let $x\in \real^p$ and $\xt\in \real^p$, if \[h(x,\xt)=\prod_{i=1}^pg_i(x_i)g_i(\xt_i)\], then \[h(x,\xt)=h((x,\xt)_{\text{swap}(S)})\]
\paragraph{Proof}
\begin{equation}
\begin{split}
    h((x,\xt)_{\text{swap}(S)})&=\prod_{\forall i\notin S}g_i(x_i)g_i(\xt_i)\prod_{\forall j\in S}g_j(\xt_j)g_j(x_j)\\
    &=\prod_{\forall i\notin S}g_i(x_i)g_i(\xt_i)\prod_{\forall j\in S}g_j(x_j)g_j(\xt_j)\\
    &=\prod_{i=1}^p g_i(x_i)g_i(\xt_i)\\
    &=h(x,\xt)
\end{split}
\end{equation}
\subsection{Lemma 2}
Let $x\in \real^p$ and $\xt\in \real^p$, and $h(x,\xt)=\sum_j h_j(x,\xt)$ and $\ \forall j$ $h_j(x,\xt)=h_j((x,\xt)_{\text{swap}(S)})$, then, $h(x,\xt)=h((x,\xt)_{\text{swap}(S)})$.
\paragraph{Proof}
\begin{equation}
\begin{split}
    h((x,\xt)_{\text{swap}(S)})&=\sum_j h_j((x,\xt)_{\text{swap}(S)})\\
    &=\sum_j h_j(x,\xt)\\
    &=h(x,\xt)
\end{split}
\end{equation}

\subsection{Theorem}

Let us denote $X=(X_o,X_m)$ and $\Xt=(\Xt_o,\Xt_m)$ resulting from the algorithm 
\[(X,\Xt)=^d(X,\Xt)_{\text{swap}(S)}\]
\paragraph{Proof}
\begin{equation}
\begin{split}
    P_{\Xt_o,\Xt_m,X_o,X_m,\hat{Z}}(\xt_o,\xt_m,x_o,x_m,\hat{z})&=
    P_{\Xt_o\mid \hat{Z}}(\xt_o;\hat{z})
    P_{\Xt_m\mid \hat{Z}}(\xt_m;\hat{z})
    P_{X_m\mid \hat{Z}}(x_m;\hat{z})
    P_{X_o\mid \hat{Z}}(x_o;\hat{z})
    P_{\hat{Z}}(\hat{z})\\
    &=
    P_{X_o\mid Z}(\xt_o;\hat{z})
    P_{X_m\mid Z}(\xt_m;\hat{z})
    P_{X_m\mid Z}(x_m;\hat{z})
    P_{X_o\mid Z}(x_o;\hat{z})
    P_{\hat{Z}}(\hat{z})\\
    &=\prod_{i=1}^pP_{X_i\mid Z}(x_i;\hat{z})P_{X_i\mid Z}(\xt_i;\hat{z})P_{\hat{Z}}(\hat{z})
    % P_{\Xt\mid X,Z}(\xt;x,z)P_{X\mid Z}(x;z)P_Z(z)\\
    % =P_{\Xt\mid Z}(\xt;z)P_{X\mid Z}(x;z)P_Z(z)\\
    % =P_{\Xt_o\mid Z}(\xt_o;z)P_{\Xt_m\mid Z}(\xt_m;z)P_{X_o\mid Z}(x_o;z)P_{X_m\mid Z}(x_m;z)P_Z(z)
\end{split}
\end{equation}
\newpage
where we used $\Xt_o\indep \Xt_m,X_o,X_m \mid \hat{Z}$,
$\Xt_m \indep X_o,X_m \mid \hat{Z}$, 
$X_m\indep X_o \mid \hat{Z}$, and $P_{X,\hat{Z}}(x,\hat{z})=P_{X,Z}(x,\hat{z})$. 
\begin{equation}
\begin{split}
    P_{X,\Xt}(x,\xt)&=\sum_{\hat{z}}P_{\Xt_o,\Xt_m,X_o,X_m,\hat{Z}}(\xt_o,\xt_m,x_o,x_m,\hat{z})\\
    &=\sum_{\hat{z}}h_{\hat{z}}(x,\xt)\\
    &=\sum_{\hat{z}}\prod_{i=1}^pg_i(x_i)g_i(\xt_i)\\
    &= P_{X,\Xt}((x,\xt)_{\text{swap}(S)}))
\end{split}
\end{equation}

where we used Lemma 1 and 2 with $g_i(x_i)\defeq P_{X_i\mid Z}(x_i;\hat{z}) P_{\hat{Z}}(\hat{z})^{0.5}$, $h_{\hat{z}}(x,\xt)\defeq P_{\Xt_o,\Xt_m,X_o,X_m,\hat{Z}}(\xt_o,\xt_m,x_o,x_m,\hat{z})$



==> chap1/miss/tex/contr.tex <==
\section{Discussion}

In this work, we have shown how to impute the missing values while preserving the guarantees of the model-x knockoffs method. We have proved that posterior imputation allows using the existing knockoffs setups without changing them in the missing data setting. The second method we introduced, univariate sampling is an alternative that allows using model-x knockoffs with missing values when the posterior sampling is not available. Moreover, we also shown how the computational requirements can be reduced when the imputation and the knockoff sampling are done jointly. To do that we have have modified two latent variable knockoff samplers to work with missing values while preserving the FDR. 

% Our experiments also demonstrate that FDR control is possible under the knockoffs methodology even when missing values are imputed.
% In the simulations,
% conducted for validating our theoretical findings
% we first investigated the bivariate affect of correlation and missing data mount on the statistical power and FDR. Next, through the constant power contours we have quantified the amount of additional data required for mitigating the affects of missing values.

% Our experiments show that FDR control is possible under the knockoffs methodology even when missing values are imputed. We have demonstrated that under different amounts of missing values, observations, and two different families of distributions.

% We have shown that posterior imputation allows using an existing knockoffs pipeline without a change in the missing values directly. As an alternative we introduced univariate sampling 

==> chap1/miss/tex/def_post.tex <==
\section{Missing Values and Knockoffs}

Let us define sets $o\subseteq\{1,\dots,p\}$ and $m=\{1,\dots,p\}\setminus o$ which represent the indices of the observed and missing R.Vs respectively. Let $X_o$ and $X_m$ denote the observed and missing random vectors respectively.

Imputation problem can be framed as a prediction problem where an estimate of the missing values $\hat{X}_m$ is given by

\[\hat{X}_m= g(X_o)\]

where $g(\cdot):\real^{|o|}\rightarrow \real^{|m|}$

Let $X=(X_o,X_m)^T$ denote the random vector without the missing values, and $\hat{X}=(X_o,\hat{X}_m)^T$ denote the imputed one. Even if $P_X$ is known and a corresponding knockoff generation algorithm exists, the algorithm doesn't generate valid knockoffs for $\hat{X}$ general as $\hat{X}\neqd X$ doesn't hold in general.

In this work, we introduce a method which allows reusing the existing knockoff samplers under the missing data scenario. 

% which works with all readily available 

% introduce a simple and general method for sampling knockoffs 
\subsection{Knockoffs for Posterior Sampled Missing Values}

% The idea behind the first algorithm is simple, 
The knockoffs framework assumes that the input distribution $P_X$ is known or known to a certain accuracy. That information can be used for imputation in such a way that the FDR control is maintained. The idea is if we can sample $\hat{X}_m$ from the posterior distribution $P_{X_m\mid X_o}$ than the joint distribution of $\hat{X}$ will remain unchanged. More importantly existing knockoff samplers can be used with the same FDR guarantee. 


% \begin{algorithm}[H]\label{alg:main}
% \caption{Posterior sampled missing value knockoffs}
%     Input: $x_o, P_X, \mathcal{A}$\\
%         % \SetAlgoLined
%             $\hat{x}_m\sim P_{X_m\mid X_o}(\cdot;x_o)$ \\
%             $x_c\leftarrow(x_o,\hat{x}_m)$\\
%             $\xt \sim \mathcal{A}(x_c,P_X) $\\
%     Output: $x_c,\xt$
% \end{algorithm}
\begin{algorithm}[H]
\caption{Posterior sampled missing value knockoffs}\label{alg:main}
 \textbf{Input:}  $x_o, P_X, \mathcal{A}, m, o$
\begin{algorithmic}
            \State $\hat{x}_m\sim P_{X_m\mid X_o}(\cdot;x_o)$
            \State  $x_c\leftarrow(x_o,\hat{x}_m)$
            \State$\xt \sim \mathcal{A}(x_c,P_X) $
\end{algorithmic}
\textbf{Output:} $x_c,\xt$
\end{algorithm}

        


% We're interested in generating $\Xt$ that is pairwise exchangeable   
% In a particular sample, 

% In \cite{} a lower bound for the computational complexity of a valid knockoff generation and metropolis-hasting based approach is introduced which also works with arbitrary distributions but requires the  

% Both algorithms that work with general distributions and distribution specific pairwise exchangeable 
% There are existing algorithms for generating pairwise exchangeable knockoffs given $P_X$. 


==> chap1/miss/tex/exp.tex <==
% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[width=.8\linewidth]{img/mvn/contr.png}
%     \caption{Constant power contours of the posterior imputation knockoffs (Algorithm \ref{alg:main}). The missing value positions are restricted to true features on the \emph{left}, to null features on the \emph{middle}, and are not restricted on the \emph{right}. Each cross is a searched pair. X axis is $\rho$ and y axis is $p_0$. Interpolation is used to to draw the constant power lines.}
%     \label{fig:mvn1}
% \end{figure*}
\section{Simulation Experiments}\label{setup}

% To investigate the effect of missing values in the knockoffs framework, we conducted various simulations. 
Because of the difficulty of obtaining ground truth variables in real world datasets simulation studies are commonly used in the model-x knockoffs literature \cite{candesPanningGoldModelX2017,barberControllingFalseDiscovery2015a,nguyenAggregationMultipleKnockoffs2020}. We’re currently working on applications in genomics datasets with missing values which require domain specific treatments and interpretation. Therefore, we have found it not suited to the scope of this paper. 

In our experiments, we have investigated the effect of missing values in the knockoffs framework by simulating a variable selection problem in different settings. The simulations are divided into two categories based on the probability distribution of the exploratory variables, namely multivariate normal (MVN) distributed and HMM distributed simulations.



% varied the number of missing values, the correlation among the variables, and the missing data pattern. 

% Moreover in this setting, we also compared our imputation methods with methods that do not come with FDR guarantees. Finally, we observed the joint effect of changing the number of samples and the number of missing values when the data is distributed according to an HMM. 

\textbf{Simulation Setup, Response Distribution:} Throughout our experiments, we have followed the simulations of \cite{sesiaGeneHuntingHidden2019} and used a Logistic Regression model as the response conditional distribution. In our simulations, we have also simulated missing data in the exploratory variables. Let $X$ be a random vector with a specified $P_X$, $\beta^{*}\in \real^p$ and $\sigma$ denotes the sigmoid function. The response variable is given by:
\[Y\sim \text{Bernoulli}(p=\sigma(X^T\beta^{*})), \quad \text{\quad }\beta^{*}_i=
\begin{cases}
    a,&\text{if } i\in S^*\\0,              &\text{otherwise}
\end{cases}\]

% \[Y\sim \text{Bernoulli}(p=\sigma(X^T\beta^{*}))\]

% where 
% \[\beta^{*}_i=
% \begin{cases}
%     a,&\text{if } i\in S^*\\0,              &\text{otherwise}
% \end{cases}
% \]

where $a$ denotes the amplitude of the coefficient and $S^*$ denotes the indices of the subset of covariates with non-zero coefficient. The $|S^*|$ is an experiment parameter and elements of $S^*$ are randomly selected from $\{1,\dots,p\}$ with equal probability and kept the same for different trials.

\textbf{Missing Values:} After generating N i.i.d samples from $\{X^{(i)}\}_{i=1}^N$, from $P_X$, we simulate missing completely at random as follows:
% mask only the non-zero coefficient covariates to simulate missing values i.e.
\begin{equation*}
    \begin{split}
        &\epsilon_j^{(i)} \sim \text{Bernoulli}(p=1-p_0) \quad j=1,\dots,p\\
        &o^i=\{j:\epsilon_j^{(i)}=1, \ j \in M\}
    \end{split}
\end{equation*}
% \[X'_i=
% \begin{cases}
%     \text{missing},&\text{if } i\in M \ \text{and}\ \epsilon_i=1\\    
%     X_i, &\text{otherwise}
% \end{cases}\]

where $M\subseteq\{1,\dots,p\}$ denotes the position of the missing values and $p_0$ denotes the probability of observing a missing value. The N i.i.d samples of observed variables and the response variables i.e. $\{X_{o^i}^{(i)},Y^{(i)}\}_{i=1}^N$ are then used as the input to the knockoffs procedure. Please refer to App. \ref{app:knock} for the knockoff setup and statistical learning algorithm used.
% is a simulation parameter, $\epsilon_i \sim \text{Bernoulli}(p=p_0)$, and $\{e_i\}_{i=1}^p$ are i.i.d.

% N i.i.d samples $\{X'^{(i)},Y^{(i)}\}_{i=1}^N$ are drawn after specifying $P_X$ and used as the input to the knockoffs procedure. 
% As the score estimator the absolute value of the coefficients of a logistic regression model with $l_1$ regularization is used. For the multivariate normal data each time $\lambda$ is selected using 5-fold-cross-validation with area under the curve metric and search space $\{1e-10,1e-2,1e-1,1,1e1\}$ is used. For HMM $\lambda$ is fixed to 1. 




% $\lambda$ is selected using 5-fold-cross-validation with area under the receiver operating curve (AUC) metric and search space $\{1e-10,1e-2,1e-1,1,1e1\}$ is used.

==> chap1/miss/tex/exp_hmm.tex <==
% \clearpage
\subsection{HMM simulations: Compensating Missing Values}

As the knockoffs method supports an arbitrary $P_X$ so does the missing value knockoffs. To show that, in this simulation we used an HMM distribution which also has applications in modeling the distribution of genetic markers in the human genome \cite{sesiaGeneHuntingHidden2019}. Our second goal was to quantify the affect of changing the missing value amount $p_0$ and the observation amount $N$ simultaneously. To observe that in detail we have done a fine grid search with parameter spaces $p_0=\{0,0.05,\dots,0.5\}$ and $N=\{500,625,750,\dots,2000\}$. We also increased number of simulation repetitions to 128 for a clearer picture of the performance. The HMM distribution is specified following the simulations in \cite{sesiaGeneHuntingHidden2019}. The emission and trasmission matrices are given in Appendix \ref{app:hmm}. Before using the exploratory variables for simulating the response variable to shift their values around to zero we subtract $4$ as in \cite{sesiaGeneHuntingHidden2019}. We have restricted the missing values to true indices and the remaining experiment parameters are given as: $p=1000$, $a=0.32$, $\mid S\mid =60$. 
% (S6.1)
% We have varied the $p_0=\{0,0.05,\dots,0.5\}$, $N=\{500,625,750,\dots,2000\}$ and recorded the average power and FDR.
% For each pair, data generation is repeated 128 times to obtained average values. 

We have only tested posterior imputation (Algorithm \ref{alg:main}) in this setting and used the Sesia HMM Knockoffs \cite{sesiaGeneHuntingHidden2019} for sampling the knockoffs. We refer to this combination as posterior sampling + Sesia HMM. HMM structure allows sampling from $P_{X_m\mid X_o}$ by first sampling from $P_{Z\mid X_o}$ then sampling from $P_{X_m\mid Z}$. We also compared Algorithm \ref{alg:main} with our modified Sesia HMM Knockoffs (Algorithm \ref{alg:sesia}). 
% Posterior probability sampling is done as described in Appendix \ref{post_hmm}. 



==> chap1/miss/tex/exp_mvn.tex <==
% \clearpage
\subsection{MVN Simulations: Correlation and Missing Values}
% $\Sigma_{ij}=\rho^{|i-j|}$
In the MVN simulations, our goal was to observe how the amount the missing data and the correlation among the exploratory variables affected the performance of the developed missing value knockoffs methods. For that reason, following \cite{barberControllingFalseDiscovery2015a,nguyenAggregationMultipleKnockoffs2020} we have used a zero-mean MVN with a special correlation matrix $\Sigma$ whose i'th row and j'th column of $\Sigma$ is given by
$\Sigma_{ij}=\rho^{|i-j|}$. By that we're able to control the correlation amount with a single parameter $\rho\in(0,1]$. 

we didn't restrict the location ($M=\{1,\dots,p\}$). In each experiment setting, we have searched the grid of different missing value amounts ($p_0=\{0,0.1,\dots,0.4\}$), and correlation values ($\rho=\{0,0.1,\dots,0.8\}$) to investigate the bivariate relationship. 

% Another question we had was whether where the missing value occurs effected the performance. For that reason we used three different missing value configurations. In the first and the second experiments the missing values are restricted to occur at the true variables ($M=S^*$) and the null variables ($M=\{1,\dots,p\}\setminus S^*$) respectively. 
% While in the third experimental setting 
% \begin{itemize}
%     \item Experiment 1: At true covariates, $M=S^*$
%     \item Experiment 2: At null covariates, $M=\{1,\dots,p\}\setminus S^*$
%     \item Experiment 3: No restrictions, $M=\{1,\dots,p\}$
% \end{itemize}

% In this simulation category we have used a MVN distribution for the exploratory variables i.e. $X\sim N(0,\Sigma)$. Following \cite{barberControllingFalseDiscovery2015a,nguyenAggregationMultipleKnockoffs2020} to probe the effect of correlation on the performance we have parametrized the covariance matrix s.t. the correlation between two variables gets lower as their positional distance increase i.e. $\Sigma_{ij}=\rho^{|i-j|}$ where $\rho\in(0,1]$ controls the correlation amount. 


% In the MVN simulations, we investigated how the correlation of the exploratory variables and the missing data amount affected variable selection. We also explored what happens to the performance when the missing data occurs only in the true variables or only in the nulls variables. Another comparison we made was between the readily available imputation methods that do not guarantee FDR control under the knockoffs framework and the methods we introduced.


% we have used the below multivariate normal (MVN) distribution where .

% \[X\sim N(\mu,\Sigma)\]

% \[\ \text{where} \quad \Sigma= \begin{bmatrix}
% \rho^0 & \rho^1 & \dots & \rho^{p-1}\\
% \rho^1 & \rho^0 & \dots & \rho^{p-2}\\
% \vdots & \vdots & \dots & \vdots\\
% \rho^{p-1} & \rho^{p-2} & \dots & \rho^{0}\\
% \end{bmatrix}, \quad \mu=0 \]

%exp. parameters
Other experimental parameters we selected are as follows: we have used $p=700$ different exploratory variables and set $N=1050$ which is slighly higher than $p$. Six \% of the variables are selected as true i.e. $\mid S\mid =42$ and the effect size is set to $a=10/ \sqrt{N}=0.38$. Each setting in the grid is repeated 31 times to obtain empirical averages. For the knockoff samplers required in Algorithm \ref{alg:main} and Appendix Algorithm \ref{alg:uni} we have used the Model-x MVN knockoffs introduced in \cite{candesPanningGoldModelX2017} which requires solving a convex optimization problem. To sample from the posterior distribution $P_{X_m\mid X_o}$(as required in Algorithm \ref{alg:main}), we have used the exact inference formulas for the the MVN distribution.
 
%  We have explored three different missing value configurations. The locations where missing values can occur are as follows:

% We have used the experiment parameters $p=700$, $a=0.38$, $\mid S\mid =42$.  but kept $N=1050$. Experiments are repeated 31 times. 




% Posterior probability distributions of MVNs used in Algorithm 1 have a closed-form solution (but it requires matrix inversion).

%different variations


% \input{tex/results_mvn_p700}

\begin{figure}
    \centering
    \includegraphics[width=.9\linewidth]{3.png}
    \caption{Heatmap of power on the left, FDR on right. The posterior imputation + MVN Knockoffs is used. Y axis changes the missing value amount ($p_0$) and x axis the correlation amount ($\rho$). FDR is generally controlled $<0.1$.
    }
    % Increasing the amount of correlation and missing values
    % On the left darker red (blue) indicates higher (lower) power. On the right values above $q=0.1$ are red and below are blue.}
    \label{fig:mvn_double}
\end{figure}

==> chap1/miss/tex/intro_new.tex <==
\section{Introduction}
Coping with increasing number of variables, optimizing predictive performance, and selecting among candidate scientific hypothesis are all valid reasons for using a variable selection algorithm. Another reality of today's datasets are missing values. Although there are existing methods for handling the missing values if applied directly, they can interfere with the assumptions of variable selection algorithms. 

In this work, we will discuss how model-x knockoffs \citep{candesPanningGoldModelX2017}, a new approach in principled variable selection, can be applied to datasets that contain missing values. By principled variable selection we refer to algorithms that aims to identify the Markov Blanket (MB) of a response variable \citep{tsamardinosPrincipledFeatureSelection2003} while providing a control of the false selections. Identifying the MB is by definition optimal as the MB refers to the smallest subset of variables that is sufficient to describe the conditional distribution of the response variable. Controlling the false selections refers to limiting the variables that are selected due to random chance and is especially important in applications where a selected variable corresponds to a scientific discovery. 

% Model-x knockoffs framework is intended for principled variable selection as it provide a false selection relevant to MB discovery without making assumptions of the response conditional distribution.

Model-x knockoffs provides a framework for repurposing existing statistical/machine learning feature scorers for MB discovery. 
% It's flexibility follows from the absence of restrictions on the conditional distribution of the response variable. 
    When the assumptions of the model-x framework holds, the expected fraction of selections that are conditionally pairwise independent with the response variable is controlled. Formally given exploratory variables $X_1,\dots, X_p$ and a response variable $Y$, let $X_{-j}=\{X_l:l\neq j\}$ denotes the variables except $X_j$, then the conditionally pairwise independent variables set is given by $\mathcal{H}_0:\{j:Y\indep X_j \mid X_{-j}\}$ \citep{candesPanningGoldModelX2017}. Given the resulting subset $\hat{S}\subseteq \{1,\dots,p\}$ from the procedure, the False Discovery Rate (FDR) \citep{benjaminiControlFalseDiscovery2001} is controlled at a selected level $q$ i.e.  
    \begin{equation}\label{eq:fdr}
        \E\bigm[\dfrac{\bigm|\hat{S}\ \cap \ \mathcal{H}_0\bigm|}{\text{max}(1,\bigm|\hat{S}\bigm|)}\bigm]\leq q
    \end{equation}
Moreover, under widely used assumptions in the probabilistic graphical models literature, that is equivalent to controlling the expected fraction of selections that are outside of the MB of the response \citep{candesPanningGoldModelX2017}. 
% As an alternative assumption, we also show that strict positiveness of the joint distribution is sufficient in the Appendix Theorem \ref{thm:mb}. 

% In the model-x knockoffs methodology, a Random Variable (R.V.) $X_j$ is a false selection if it's conditionally independent of the response variable $Y$ given the remaining exploratory variables $X_{-j}=\{X_l:l\neq j\}$ i.e. $Y\indep X_j \mid X_{-j}$. When the assumptions of the model-x framework holds, the expected fraction of selections that are false is controlled at a desired level. Formally let $\mathcal{H}_0:\{j:Y\indep X_j \mid X_{-j}\}$ denotes set of false selection and $\hat{S}\subseteq \{1,\dots,p\}$ denotes the set of selections, the False Discovery Rate (FDR) \citep{benjaminiControlFalseDiscovery2001} is controlled at a selected level $q$ i.e.  \[ \E\bigm[\dfrac{\bigm|\hat{S}\ \cap \ \mathcal{H}_0\bigm|}{\text{max}(1,\bigm|\hat{S}\bigm|)}\bigm]\leq q\]

% In \citep{candesPanningGoldModelX2017}, it's stated that 
% For the model-x knockoffs to be used for MB discovery 
% The set of false selections under 
% The false selections of the model

% One assumption of the model-x knockoffs is the accurate knowledge of the distribution of the exploratory variables and the imputation of the missing values can alter the distribution. To describe the problems imputation can cause, we briefly review how the exploratory variable distribution is used in the knockoffs framework.

% Next, the concatenated matrix $[\Xb, \Xtb]$ is inputted to a feature scorer to obtain $W_j([\Xb, \Xtb])$. Finally 

% $\mathcal{A}$ i.e. $\Xt^{(i)} \sim \mathcal{A}(X^{(i)},P_X)$ s.t. $\Xt^{(i)}$ and $X^{(i)}$ are pairwise exchangeable. 


Model-x frameworks requires the following two assumptions to hold for the FDR control. The first assumption is the pairwise exchangeability of $\Xb$ and $\Xtb$. The second assumption is the independence of the rows of the concatenated matrix $[\Xb, \Xtb]$ i.e.
$X^{(i)},\Xt^{(i)} \indep X^{(j)},\Xt^{(j)}$. In practise to give the FDR guarantees those assumptions needs to be justified.

% There are two critical assumptions that model-x knockoffs make for maintaining those guarantees. The first is the \pe between the ``knockoff'' matrix $\Xtb\in\real^{N\times p}$ and the original exploratory variable matrix $\Xb\in\real^{N\times p}$. The second assumption is the independence of the rows of the concatenated matrix $[\Xb,\Xtb]$. In practise to give the FDR guarantees those assumptions needs to be justified.

A frequently occurring problem in practise is missing data and it has the potential to effect those assumptions. Because statistical learning algorithms do not support missing data (in general) imputation is applied. The matrix with filled missing values $\hat{\Xb}$ in general doesn't have the same distribution with $\Xb$ and even its rows can be dependent.

To the best of our knowledge the effect of missing data on the assumptions model-x knockoffs has not been discussed previously. In this paper, we will first formulate those nuances and next show the existing assumptions of the model-x framework enables rigorous imputation of missing values.

In Section 2, we give the necessary background regarding model-x knockoffs and missing data imputation. In Section 3, we  introduce imputation methods that preserves the theoretical guarantees. In Section 4, we discuss how the certain latent variable models enables efficient sampling of knockoffs and imputation. In Section 5, simulations will be used to demonstrate our theoretical findings.
% The two critical assumptions that model-x knockoffs make f
% The assumptions of the model-x knockoffs for FDR control can be violated after missing values are imputed. Formally, given the observed variables $X_{o^i}^{(i)}=\{X_i:i\in o^i\}$ where $o^i\subseteq\{1,\dots,p\}$ and $m^i=\{1,\dots,p\}\setminus o^i$ an imputation method outputs the imputed variables $\hat{X}_{m^i}^{(i)}$. The resulting imputed matrix is denoted by $\hat{\Xb}$ where the i'th row is denoted by $\Xh^{(i)}$ and $\Xh^{(i)}_{o^i}=X^{(i)}_{o^i}$. We use $o$ and $m$ instead of $o^i$ and $m^i$ if there is no ambiguity. To understand the effect of imputation  we categorized imputation methods into three:

% \begin{enumerate}[label=\roman*]
%   \item $(\hat{X}_{m^1}^{(1)},\dots, \hat{X}_{m^N}^{(N)}) = g(X_{o^1}^{(1)},\dots,X_{o^N}^{(N)})$
%   \item $\hat{X}_{m}^{(i)}= g(X_{o}^{(i)})$
%   \item $\hat{X}_{m}^{(i)}= g(X_{o}^{(i)},\epsilon)$ where $\epsilon$ denotes an independent R.V.
% \end{enumerate}

% if the knockoffs are sampled using the pre-imputed distribution $P_X$ because it only guarantees pairwise exchangeability of 

% i.e. $\Xt^{(i)} \sim P_{\Xt\mid X}(\cdot;\Xh^{(i)})$, in general $\hat{\Xb}$ and $\Xb$ won't be pairwise exchangeable.

% to satisfy the  should be sampled using the distribution of the imputed vector $P_{\Xh}$ instead of $P_X$.

% An example to case ii) can be mean imputation $g(x_o)=\mu_m$, or a linear regression model $g(x_o)=w^Tx_o$. Similarly, iii) can be 
% In case ii) and iii) if the function $g(\cdot)$ is estimated from a different dataset, the independence of the rows will be preserved. 


% because the function $g(\cdot)$ changes the dependence between $\Xhat_m$ and $$


% In general the joint distribution of the observed and imputed random vectors is not equal to the joint distribution of the fully observed random vector i.e. $(X_{o}^{(i)},\hat{X}_{m}^{(i)})\neqd (X_{o}^{(i)},X_{m}^{(i)})$ where $m=\{1,\dots,p\}\setminus o$. Therefore, if one samples the knockoff for the imputed vector using the original distribution $P_X$ in general the pairwise exchangeability would not hold. To sample valid knockoffs the joint distribution of $\hat{X}^{(i)}=(X_{o}^{(i)},\hat{X}_{m}^{(i)})$ needs to be known accurately and that leads to two problems. First, deriving $P_{\hat{X}^{(i)}}$ using $P_{X}$ might not be practical for all functions $g(\cdot)$ and second even if the derivation is possible sampling valid knockoffs for the new distribution might not be tractable.

% A simple solution to this problem is would be keeping  $P_{\hat{X}^{(i)}}$ equal to $P_{X}$. Once that is done any knockoff sampler that works for $P_{X}$ will also work for the imputed vector $\hat{X}^{(i)}$. That is very practical as the existing code written for sampling knockoffs can be used directly with the imputed data. In this work we introduce a imputation algorithm that preserves the input distribution. 

Our contributions in this paper are: 

\begin{itemize}
    \item Formulating the effects of the missing data imputation on the model-x framework
    \item Proving posterior sampled imputation allows reusing existing knockoffs samplers
    \item Proposing an univariate method that doesn't require posterior sampling
    \item Showing knockoff sampling can be jointly done with imputation
    % \item Quantifying the joint effect of correlation and missing data on power
    % \item Describing the trade-off between the number of missing data and observations
\end{itemize}

% The imputation method estimates the missing variables $X_{m}^{(i)}$ using the observed variables $X_{o}^{(i)}$ where $o\subseteq\{1,\dots,p\}$ and $m=\{1,\dots,p\}\setminus o$ represents the indices of the observed and missing R.Vs. Formally, the estimate is denoted as $\hat{X}_{m}^{(i)}= g(X_{o}^{(i)})$ where $g(\cdot):\real^{|o|}\rightarrow \real^{|m|}$ is the prediction function. The distribution of $X_o,\hat{X}_m)^T$ denote the imputed one.

% If only a subset of the variables in the i'th row denoted with $o^{(i)}\subseteq\{1,\dots,p\}$ are observed, 
% \{1,\dots,p\}\setminus o$ of the variables in the i'th row is 

 
% Imputation problem can be framed as a prediction problem where an estimate of the missing values $\hat{X}_m$ is given by



% $\xt \sim \mathcal{A}(x_c,P_X) 

% Model-x knockoffs framework 


% Variable selection algorithms are used for coping with

==> chap1/miss/tex/latent_gz_2.tex <==

In Algorithm \ref{alg:gz}, we have extended the GZ knockoff sampler \cite{gimenezKnockoffsMassNew2019} to the missing data setting. GZ knockoff sampler supports a broader class of latent variable models than the HMM sampler as it doesn't require $P_{Z}$ to form a Markov Chain. Compared to the original, the modified algorithm restricts the order of sampling to first $Z'$ and then $\Xt$. Moreover, just as in the HMM case it has two additional steps: sampling from the posterior and imputing the missing values. We denote $Z_{k:l}=\{Z_i: i\geq k \ \& \ i\leq l\}$.

\begin{algorithm}[H]
\caption{Modified GZ Knockoffs}\label{alg:gz}
\begin{algorithmic}
\STATE {\bfseries Input:} $x_o, P_Z, P_{X\mid Z}, m, o$
\STATE  $\zh \sim P_{Z\mid X_o}(\cdot;x_o)$\hfill\COMMENT{Posterior Sampling with $X_o$} 
\STATE  $\xh_m \sim P_{X_m\mid Z}(\cdot;\zh)$ 
\hfill\COMMENT{Imputing Originals} 
\FOR{\texttt{$i=1,\dots,L$}}
\STATE  $z'_i \sim P_{Z_i\mid X,Z_{i+1:L},Z_{1:i-1}}(\cdot;\xh,\hat{z}_{i+1:L},z'_{1:i-1})$
% \quad i=1,\dots,L$ 
\ENDFOR
\STATE  $\xt_m \sim P_{X_m\mid Z}(\cdot;z')$
\STATE  $\xt_o \sim P_{X_o\mid Z}(\cdot;z')$
\STATE {\bfseries Output:}  $\hat{x}, \xt$ 
\end{algorithmic}
\end{algorithm}

% Let $\xh\in \real^p$ where $\xh_m\in \real^m$ denotes the estimated missing values and $\xh_o=x_o$.


% \begin{equation}
%     \begin{split}
%         &\zh \sim P_{Z\mid X_o}(\cdot;x_o)\\
%         &\xh_m \sim P_{X_m\mid Z}(\cdot;\zh)\\
%         % &z' \sim \text{GZ}(\zh,x_o,\xh_m)\\
%         % &z'_i \sim P_{Z_i\mid X, Z}(\zh,x_o,\xh_m)\\
%         &z'_i \sim P_{Z_i\mid X,Z_{i+1:L},Z_{1:i-1}}(\cdot;\xh,\hat{z}_{i+1:L},z'_{1:i-1})\\
%         &\xt_m \sim P_{X_m\mid Z}(\cdot;z')\\
%         &\xt_o \sim P_{X_o\mid Z}(\cdot;z')
%     \end{split}
% \end{equation}

% \begin{equation}
% \begin{split}
%     P_{\hat{X},\Xt,Z'}(\xh,\xt,z') &= P_{\Xt_o\mid Z'}(\xt_o; z')P_{\Xt_m\mid Z'}(\xt_m\mid z')\sum_{\zh}P_{Z'\mid \Zh,X_o,\Xh_m}(z';\zh,x_o,\xh_m)P_{X_o,\Xh_m,\Zh}(x_o,\xh_m,\zh)\\
%     &y=P_{\Xt_o\mid Z'}(\xt_o; z')P_{\Xt_m\mid Z'}(\xt_m\mid z')\sum_{\zh}P_{Z'\mid \Zh,X_o,\Xh_m}(z';\zh,x_o,\xh_m)P_{X_o,X_m,\Zh}(x_o,\xh_m,\zh)\\
% \end{split}
% \end{equation}

\begin{cor}\label{thm:gz}
% Let $\Xh$ denote the imputed $X$, and $\Xt$ its knockoff. 
Let $X\sim P_X$ and $P_X$ can be denoted as a latent variable model i.e.
\begin{equation*}
    \begin{split}
        &Z \sim P_Z \\
        &X_j\mid Z \sim P_{X_j\mid Z}(\cdot;Z) \quad j=1,\dots,p
    \end{split}
\end{equation*}

where $Z$ is a $L$ dimensional random vector. We assume the distribution $P_{X,R}$ satisfies MCAR or MAR. If $\Xh$ and $\Xt$ are resulting from Algorithm \ref{alg:gz}, then $\Xh$ and $\Xt$ are pairwise exchangeable.
% $\forall \ S\subseteq \{1,\dots,p\}$
% \[(\Xh,\Xt)_\swap\eqd\Xh,\Xt\]
% Let $\Xh:\Omega\rightarrow{\real^p}$ be a random vector and $\Xh_o=X_o$,

\end{cor}

The proof is in Appendix \ref{app:gz}



==> chap1/miss/tex/latent_sesia.tex <==
\section{Jointly Imputing and Knockoff Sampling in Latent Variable Models}

% We have introduced a method for reusing existing sampler. 

In the preceding section, we have treated imputation and knockoff sampling as two different stages and shown how that enables reusing existing knockoff samplers. In this section, we will show how jointly imputing and knockoff sampling can have computational advantages in latent variable models. The intuition is in certain latent variable models posterior imputation and knockoff sampling requires two separate samples from the latent variable posterior distribution and  we can actually reduce that to one sample by modifying the knockoff sampler. The next theorem illustrates that:

\begin{thm}\label{thm:latent}
% Let $X\sim P_X$ where $P_X$ is a Hidden Markov Model
Assume $X,Z \sim P_{X,Z}(\cdot,\cdot)$ and 
$P_{Z',\Xt \mid \Zh}(z',\xt;\zh)$ is a probability distribution s.t. resulting $X$ and $\Xt$ are \pe when the following sampling is used:
\begin{equation*}
    \begin{split}
        &\Zh \mid X \sim P_{Z\mid X}(\cdot;X)\\
        &Z',\Xt \mid \Zh \sim P_{Z',\Xt \mid \Zh}(\cdot,\cdot;\Zh)\\
    \end{split}
\end{equation*}

Then if the missing data pattern is MAR or MNAR, and $X_m \indep X_o \mid Z$ holds, the following sampling procedure also produces $\Xh$ and $\Xt$ that are \pe:

\begin{equation*}
    \begin{split}
        &\Zh \mid \Xh_o \sim P_{Z\mid X_o}(\cdot;\Xh_o)\\
        &\Xh_m \mid \Zh \sim P_{X_m\mid Z}(\cdot;\Zh)\\
        &Z',\Xt \mid \Zh \sim P_{Z',\Xt \mid \Zh}(\cdot,\cdot;\Zh)\\
    \end{split}
\end{equation*}

where $\Xh=(\Xh_1,\dots,\Xh_p)^T$ denote the imputed vector and $\Xh_o=X_o$.
% $\forall \ S\subseteq \{1,\dots,p\}$
% \[(\Xh,\Xt)_\swap\eqd\Xh,\Xt\]
\end{thm}
Proof is in \ref{app:latent}. This theorem shows that existing latent latent variables knockoff samplers such as HMM knockoff sampler \cite{sesiaGeneHuntingHidden2019} can be extended to the missing data setting. 

% in two different stages requires sampling from the latent variable posterior twice \footnote{One from $P_{Z\mid X_o}$, and one from $P_{Z\mid }$}. As it's possible to both tasks with a single latent variable posterior sample.

% The main idea is in certain latent variable models imputing and knockoff sampling in two different stages requires sampling from the latent variable posterior twice \footnote{One from $P_{Z\mid X_o}$, and one from $P_{Z\mid }$}. As  it's possible to both tasks with a single latent variable posterior sample.


% A different approach than the previous section which focuses on reusing existing knockoff samplers is adjusting knockoff samplers to support missing values. Latent variables models 

% In latent variable models, the posterior sampling used in 

% The posterior imputation algorithm introduced requires sampling from $P_{X_o\mid X_m}$ and as the next step 

% In the previous section we have introduced an imputation algorithm

% One can threat the missing values as latent variables and attempt to use the existing samplers for latent variables such as HMM knockoff sampler \cite{sesiaGeneHuntingHidden2019} and GZ knockoff sampler \cite{gimenezKnockoffsMassNew2019} directly. However, those samplers only guarantee the pair-wise exchangeablity of the observed variables, not the hidden variables and therefore not the imputed variables.

% We have expanded those two algorithms to support missing values. The resulting modified samplers doesn't have a theoretical advantage over Algorithm $\ref{alg:main}$ but a computational one. That is because instead of sampling from a posterior distribution twice (once for imputation once for knockoff sampling) they only sample once. 


% where the first one works for HMMs and second one for general 
% Although in 
% they won't guarantee the pair-wise exchangeablity of the imputations.

% In latent variable models, generating knockoffs is possible without using the marginal distribution of $X$. Existing knockoff samplers HMM knockoff sampler \cite{sesiaGeneHuntingHidden2019} and GZ knockoff sampler \cite{gimenezKnockoffsMassNew2019}.
% do not support missing values readily. 


% That structure can also be used for saving computations
% In the previous section we have introduced a way of reusing existing samplers. 


% It's also possible to adjust the existing knockoff samplers to do missing value imputation explicit. We have modified the existing algorithms i.e. . The advantage is it requires less computations to generate valid knockoffs. 

% Algorithm \ref{alg:main}, requires posterior sampling for imputation in case of latent variables 

% The latent variable knockoff samplers generally first do a posterior sampling from 

% This can be advantage 

% from $P_{Z\mid X_o}(\cdot;x_o)$ for imputation and later sampling $P_{Z\mid X}(\cdot;x)$ 


% imputing the missing values during the algo

% For example, for HMMs a knockoff sampler is introduced in \cite{sesiaGeneHuntingHidden2019}. 

% d for directed graphical models with certain factorization 
% instead of first imputing the 

\begin{algorithm}[H]
\caption{Modified Sesia HMM Knockoffs}\label{alg:sesia}

\begin{algorithmic}
\STATE {\bfseries Input:}  $x_o, P_{Z}, P_{X\mid Z}$,$P_{\Zt \mid Z}, m, o$\\
\STATE  $\zh \sim P_{Z\mid X_o}(\cdot;x_o)$\hfill\COMMENT{Posterior Sampling with $X_o$} 
% \For{i=1,\dots,|m|}
\STATE  $\xh_m \sim P_{X_m\mid Z}(\cdot;\zh)$\hfill\COMMENT{Imputing Originals} 
\STATE  $z' \sim P_{\Zt \mid Z}(\cdot;\zh)$
% \mathcal{A}(\zh,P_Z)$
\STATE  $\xt_m \sim P_{X_m\mid Z}(\cdot;z')$
\STATE  $\xt_o \sim P_{X_o\mid Z}(\cdot;z')$
\STATE {\bfseries Output:} $\hat{x}, \xt$ 
\end{algorithmic}
\end{algorithm}

% \begin{equation}
%     \begin{split}
%         &\zh \sim P_{Z\mid X_o}(\cdot;x_o)\\
%         &\xh_m \sim P_{X_m\mid Z}(\cdot;\zh)\\
%         &z' \sim \text{SCIP}(\zh)\\
%         &\xt_m \sim P_{X_m\mid Z}(\cdot;z')\\
%         &\xt_o \sim P_{X_o\mid Z}(\cdot;z')
%     \end{split}
% \end{equation}

We have provided the modified version of the HMM knockoff sampler \cite{sesiaGeneHuntingHidden2019} in Algorithm \ref{alg:sesia}. The only differences from the original sampler is the first two steps: sampling from the posterior and imputing the originals. We have demonstrated in Appendix Proposition \ref{thm:hmm_post} that HMM structure allows tractable sampling from the posterior $P_{Z\mid X_o}$ and provided the Algorithm \ref{alg:hmm_post}. The second step is to impute the originals using $X_{X_m\mid Z}$ and it's relatively easy as given the hidden states emission probabilities factors out.
\begin{cor}\label{thm:sesia}
% Let $X\sim P_X$ where $P_X$ is a Hidden Markov Model
If $X$ distributed according to an HMM, and we assume the distribution $P_{X,R}$ satisfies MCAR or MAR, then given $\Xh$ and $\Xt$ resulting from Algorithm \ref{alg:sesia} if $P_{\Zt \mid Z}$ is pairwise exchangeable with respect to $P_Z$ then $\Xh$ and $\Xt$ are pairwise exchangeable.

% $\forall \ S\subseteq \{1,\dots,p\}$
% \[(\Xh,\Xt)_\swap\eqd\Xh,\Xt\]
\end{cor}
Proof follows from the fact the Sesia et al. \cite{sesiaGeneHuntingHidden2019} approach is a valid knockoff sampler and HMM has $X$ is conditionally jointly independent given $Z$. The advantage of Alg. \ref{alg:sesia} lies in using the same latent variable samples to impute and sample knockoffs. Alg. \ref{alg:sesia} samples from distributions $P_{Z\mid X_o},P_{X_m\mid Z}, P_{\Zt\mid Z}$, and $P_{X\mid Z}$ in order. In addition to those four, Alg. \ref{alg:sesia} samples from $P_{Z\mid X}$. For HMMs with $p$ time steps and $L$ hidden states the total complexity of Alg. \ref{alg:sesia} and Alg. 1 are $O(2pL^2)$ and $O(3pL^2)$ respectively. Therefore, Alg. 3 reduces the complexity by one third.

% Proof is in Appendix \ref{app:sesia}

==> chap1/miss/tex/notation.tex <==
\section{Notation}
\begin{equation}
    \begin{split}
        X &: \text{A random vector with p R.Vs}\\
        P_X(x) &: \text{probability density (mass) function of random vector X} \\
        X \sim P_X(\cdot) &: \text{X is sampled with $P_X$}\\
        \mathcal{A}(x,\pin) &: \text{an algorithm with a random output}\\
        \Xt \sim \mathcal{A}(x,\pin) &: \text{$\Xt$ is sampled using algorithm $\mathcal{A}$}\\
        P_{X\mid Y}(x;y) &: \text{conditional probability density (mass) function of X given Y} \\
        X \eqd Y &: \text{equality in distribution}
    \end{split}
\end{equation}

==> chap1/miss/tex/proof_gz.tex <==
\subsection{Theorem \ref{thm:gz}}\label{app:gz}
To prove Theorem \ref{thm:gz}, we start by proving the following lemmas. For notational convenience if $k>l$ or $l<k$, $Z_{k:l}$ is omitted from a function ex: $P_{X,Z_{k:l}}(x,z_{k:l})=P_X(x)$.

% \section{Lemma}
\begin{lem}\label{lem:gz1}
Let us define:
\begin{equation*}
    \begin{split}
        g_i(\hat{z}_{i+1:T},z',x)&\defeq \sum_{\hat{z_i}}P_{Z_i\mid X,Z_{i+1:T},Z_{1:i-1}}(z_i';x,\hat{z}_{i+1:T},z'_{1:i-1})g_{i-1}(\hat{z}_{i:T},z',x), \ \forall i=2,\dots, T\\
        g_1(\hat{z}_{2:T},z',x)&\defeq\sum_{\hat{z}_1}P_{Z_1\mid X,Z_{2:T}}(z'_1;x,\zh_{2:T})P_{Z,X}(\zh,x)
        % g_T(z',x)&\defeq\sum_{\hat{z}_T}P(z'_;x,\zh_{2:T})P(\zh,x)
    \end{split}
\end{equation*}

Then, $\forall i=1,\dots, T$ and $\zh, z', x$

\[g_i(\hat{z}_{i+1:T},z',x)=P_{Z_{1:i},Z_{i+1:T},X}(z'_{1:i},\zh_{i+1:T},x)\]
\end{lem}
\begin{proof}[Proof]
Proof by induction\\
Base: $\forall \ \zh, z', x$
\begin{equation}\label{eq:lem:gz1}
\begin{split}
    g_1(\zh_{2:T},z',x)&=P_{Z_1\mid X,Z_{2:T}}(z'_1;x,\zh_{2:T})\sum_{\hat{z}_1}P_{Z,X}(\zh,x)\\
    &=P_{Z_1\mid X,Z_{2:T}}(z'_1;x,\zh_{2:T})P_{Z_{2:T},X}(\zh_{2:T},x)\\
    &= P_{Z_1,Z_{2:T},X}(z'_1,\hat{z}_{2:T},x)
\end{split}
\end{equation}

\ref{eq:lem:gz1}b follows from law of total probability. \ref{eq:lem:gz1}c follows from definition of conditional probability.

Step k: 

From step k-1, we have: $\forall \zh, z', x$
\[g_{k-1}(\zh_{k:T},z',x)=P_{Z_{1:k-1},Z_{k:T},X}(z'_{1:k-1},\zh_{k:T},x)\]

Then, $\forall \zh, z', x$
\begin{subequations}\label{eq2:lem:gz1}
\begin{align}
        g_k(\zh_{k+1:T},z',x)&=P_{Z_k\mid X,Z_{k+1:T},Z_{1:k-1}}(z_k';x,\hat{z}_{k+1:T},z'_{1:k-1})\sum_{\hat{z_k}}g_{k-1}(\hat{z}_{k:T},z',x)\\
        &=P_{Z_k\mid X,Z_{k+1:T},Z_{1:k-1}}(z_k';x,\hat{z}_{k+1:T},z'_{1:k-1})P_{Z_{1:k-1},Z_{k+1:T},X}(z'_{1:k-1},\zh_{k+1:T},x)\\
        &=P_{Z_{1:k},Z_{k+1:T},X}(z'_{1:k},\zh_{k+1:T},x)
\end{align}
\end{subequations}

\ref{eq2:lem:gz1}b follows from step k-1 and total law of probability. \ref{eq2:lem:gz1}c follows from definition of conditional probability.
\end{proof}
% \section{Lemma}
% \[\sum_{\hat{z}}P_{Z'\mid X,\hat{Z}}(z';x,\hat{z})P_{X,Z}(x,\hat{z})=g_T(z',x)
% \]
% \subsection{Proof}
% \begin{equation}
%     \begin{split}
%         \sum_{\hat{z}}P_{Z'\mid X,\hat{Z}}(z';x,\hat{z})P_{X,Z}(x,\hat{z})
%         &=
%         \sum_{\hat{z}} P_{X,Z}(x,\hat{z}) \prod_{i=0}^{T-1}P_{Z'_{T-i}\mid X,\hat{Z},Z'_{1:T-i-1}}(z'_{T-i}; x,\hat{z},z'_{1:T-i-1})\\
%         &=\sum_{\hat{z}} P_{X,Z}(x,\hat{z})\prod_{i=0}^{T-1}P_{Z_{T-i}\mid X,Z_{T-i+1:T},Z_{1:T-i-1}}(z'_{T-i}; x,\hat{z}_{T-i+1:T},z'_{1:T-i-1})\\
%         =\sum_{\hat{z}_{2:T}} [\prod_{i=0}^{T-2}P_{Z_{T-i}\mid X,Z_{T-i+1:T},Z_{1:T-i-1}}&(z'_{T-i}; x,\hat{z}_{T-i+1:T},z'_{1:T-i-1})]\sum_{\zh_1}P_{X,Z}(x,\hat{z})P_{Z_1\mid X, Z_{2:T}}(z'_1;x_1,\zh_{2:T})\\
%         &=\sum_{\hat{z}_{2:T}} [\prod_{i=0}^{T-2}P_{Z_{T-i}\mid X,Z_{T-i+1:T},Z_{1:T-i-1}}(z'_{T-i}; x,\hat{z}_{T-i+1:T},z'_{1:T-i-1})]g_1(\zh_{2:T},z',x)\\
%         &\quad \quad \dots  \\
%         &=\sum_{\zh_T}P_{Z_T\mid X,Z_{1:T-1}}(z'_{T}; x,z'_{1:T-1})g_{T-1}(\zh_{T},z',x)\\
%         &=g_T(z',x)
%     \end{split}
% \end{equation}

% The first equality follows from chain rule, second line follows from how $z'$ is sampled, in the third line all terms that depends on $\zh_1$ are grouped, fourth line comes from definition of $g_1$ and finally recursively applying the procedure 

\begin{lem}\label{lem:gz2}

Let $Z'$ sampled as in Algorithm \ref{alg:gz}, then
$\forall \ i=1,\dots,T$ and $\forall \zh, z', x$ 
\[\hspace*{-1cm}\sum_{\hat{z}_{1:i}}P_{Z'\mid X,\hat{Z}}(z';x,\hat{z})P_{X,Z}(x,\hat{z})=g_i(\zh_{i+1:T},z',x)\prod_{i=0}^{T-1-i}P_{Z_{T-i}\mid X,Z_{T-i+1:T},Z_{1:T-i-1}}(z'_{T-i}; x,\hat{z}_{T-i+1:T},z'_{1:T-i-1})\]
% \prod_{i=0}^{T-1-i}P_{Z'_{T-i}\mid X,\hat{Z},Z'_{1:T-i-1}}(z'_{T-i}; x,\hat{z},z'_{1:T-i-1})
\end{lem}
\begin{proof}

Proof by induction:

Base:$\forall \zh, z', x$ 

\begin{subequations}\label{proof:lem:gz2}
\begin{align}
% \hspace*{-1cm}
        \sum_{\hat{z}_i}P_{Z'\mid X,\hat{Z}}&(z';x,\hat{z})P_{X,Z}(x,\hat{z})\\
        &=
        \sum_{\zh_1} P_{X,Z}(x,\hat{z}) \prod_{i=0}^{T-1}P_{Z'_{T-i}\mid X,\hat{Z},Z'_{1:T-i-1}}(z'_{T-i}; x,\hat{z},z'_{1:T-i-1})\\
        &=\sum_{\zh_1} P_{X,Z}(x,\hat{z})\prod_{i=0}^{T-1}P_{Z_{T-i}\mid X,Z_{T-i+1:T},Z_{1:T-i-1}}(z'_{T-i}; x,\hat{z}_{T-i+1:T},z'_{1:T-i-1})\\
        &= [\prod_{i=0}^{T-2}P_{Z_{T-i}\mid X,Z_{T-i+1:T},Z_{1:T-i-1}}(z'_{T-i}; x,\hat{z}_{T-i+1:T},z'_{1:T-i-1})]\sum_{\zh_1}P_{X,Z}(x,\hat{z})P_{Z_1\mid X, Z_{2:T}}(z'_1;x_1,\zh_{2:T})\\
        &=g_1(\zh_{2:T},z',x)\prod_{i=0}^{T-2}P_{Z_{T-i}\mid X,Z_{T-i+1:T},Z_{1:T-i-1}}(z'_{T-i}; x,\hat{z}_{T-i+1:T},z'_{1:T-i-1})\\
\end{align}
\end{subequations}


\ref{proof:lem:gz2}b from chain law. \ref{proof:lem:gz2}c follows from definition of sampling. In \ref{proof:lem:gz2}d the only term that depends on $\zh_1$ is $P_{X,Z}$. In \ref{proof:lem:gz2}e the definition of $g_1$ is used (as defined in Lemma \ref{lem:gz1}).

Step k:$\forall \zh, z', x$ 

\begin{subequations}\label{proof:lem:gz2:2}
\begin{align}
        &\sum_{\hat{z}_{1:k}}P_{Z'\mid X,\hat{Z}}(z';x,\hat{z})P_{X,Z}(x,\hat{z})\\
        &=\sum_{\hat{z}_k}\sum_{\hat{z}_{1:k-1}}P_{Z'\mid X,\hat{Z}}(z';x,\hat{z})P_{X,Z}(x,\hat{z})\\
        &=\sum_{\hat{z}_k}g_{k-1}(\zh_{k:T},z',x)\prod_{i=0}^{T-k}P_{Z_{T-i}\mid X,Z_{T-i+1:T},Z_{1:T-i-1}}(z'_{T-i}; x,\hat{z}_{T-i+1:T},z'_{1:T-i-1})\\
        &=\prod_{i=0}^{T-k-1}P_{Z_{T-i}\mid X,Z_{T-i+1:T},Z_{1:T-i-1}}(z'_{T-i}; x,\hat{z}_{T-i+1:T},z'_{1:T-i-1})\\& \quad\sum_{\hat{z}_k}g_{k-1}(\zh_{k:T},z',x)P_{Z_{k}\mid X,Z_{k+1:T},Z_{1:k-1}}(z'_{k}; x,\hat{z}_{k+1:T},z'_{1:k-1})\\
        &=g_{k}(\zh_{k+1:T},z',x)\prod_{i=0}^{T-k-1}P_{Z_{T-i}\mid X,Z_{T-i+1:T},Z_{1:T-i-1}}(z'_{T-i}; x,\hat{z}_{T-i+1:T},z'_{1:T-i-1})
\end{align}
\end{subequations}


\ref{proof:lem:gz2:2}b follows from reordering in notation. \ref{proof:lem:gz2:2}c holds as step k-1 is assumed to hold. In step \ref{proof:lem:gz2:2}d and \ref{proof:lem:gz2:2}e only term depends on $\xh_k$ is $g_{k-1}$. In step \ref{proof:lem:gz2:2}f, the definition of $g_k$ is used (as defined in Lemma \ref{lem:gz1}).
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:gz}]

In Algorithm \ref{alg:gz}, $\Zh\sim P_{Z\mid X_o}(\cdot;X_o)$ and $\Xh_m\sim P_{X_m\mid Z}(\cdot;\Zh)$ is used. Combining Lemma \ref{lem:p_z_x} and Lemma \ref{lem:mar} we have $P_X=P_{\Xh}$ under the MAR or MCAR assumption.

We prove another required equality. $\forall \xh, \xt, z'$
\begin{subequations}\label{proof:gz}
\begin{align}
    P_{\Zh,\Xh}(\zh,\xh)&=P_{\Xh_m\mid \Zh}(\xh_m; \zh)P_{\Zh\mid X_o}( \zh;x_o)P_{X_o}(x_o)\\
    &=P_{X_m\mid Z}(\xh_m; \zh)P_{Z\mid X_o}( \zh;x_o)P_{X_o}(x_o)\\
    &=P_{X_m\mid Z}(\xh_m; \zh)P_{X_o\mid Z}(x_o;\zh)P_{Z}(\zh)\\
    &=P_{Z,X}(\zh,\xh)
\end{align}
\end{subequations}
\ref{proof:gz}a follows from chain rule and $P_X=P_{\Xh}$. \ref{proof:gz}b follows from sampling definitions. \ref{proof:gz}c follows from definition of conditional independence.
 
\begin{subequations}\label{proof:gz2}
\begin{align}
    P_{\hat{X},\Xt,Z'}(\xh,\xt,z') &= P_{\Xt\mid Z'}(\xt; z')\sum_{\zh}P_{Z'\mid \Zh,\Xh}(z';\zh,\xh)P_{\Zh,\Xh}(\zh,\xh)\\
    &= P_{X\mid Z}(\xt; z')\sum_{\zh}P_{Z'\mid Z,X}(z';\zh,\xh)P_{Z,X}(\zh,\xh)\\
    &= P_{X\mid Z}(\xt; z')g_T(z',\xh)\\
    &=P_{X\mid Z}(\xt; z')P_{Z,X}(z',\xh)\\
    &=P_Z(z')\prod_{i\in o} P_{X_i\mid Z}(\xh_i;z')\prod_{i\in m} P_{X_i\mid Z}(\hat{x}_i;z')\prod_{i=1}^p P_{X_i\mid Z}(\xt_i;z')
\end{align}
\end{subequations}


In \ref{proof:gz2}b, $P_{X\mid Z}=P_{\Xt\mid Z'}$ follows from the sampling definitions and Eq. \ref{proof:gz} is used for the joint distribution equality. In \ref{proof:gz2}c, Lemma \ref{lem:gz2} is used. In \ref{proof:gz2}d Lemma \ref{lem:gz1} and \ref{proof:gz2}e follows from the conditional independence assumption assumed in Theorem \ref{thm:gz}.

% \begin{equation}
%     \begin{split}
%         P_{\hat{X},\Xt,Z'}((\xh,\xt)_\swap,z')&=P_Z(z')\prod_{i\in o} P_{X_i\mid Z}(x_i;z')\prod_{i\in m} P_{X_i\mid Z}(\hat{x}_i;z')\prod_{i=1}^p P_{X_i\mid Z}(\xt_i;z')
%     \end{split}
% \end{equation}
\begin{alignat*}{3}
        P_{\hat{X},\Xt,Z'}((\xh,\xt)_\swap,z')&=P_{Z}(z')&&
        \prod_{i\in o\setminus S}P_{X_i\mid Z}(x_i;z')\prod_{i\in o\cap S}P_{X_i\mid Z}(\xt_i;z')\\
        & &&\prod_{i\in m\setminus S}P_{X_i\mid Z}(\xh_i;z')
        \prod_{i\in m\cap S}P_{X_i\mid Z}(\xt_i;z')\\
        & &&\prod_{i\in o\setminus S}P_{X_i\mid Z}(\xt_i;z')\prod_{i\in o\cap S}P_{X_i\mid Z}(x_i;z')
        \\
        & && \prod_{i\in m\setminus S}P_{X_i\mid Z}(\xt_i;z')
        \prod_{i\in m\cap S}P_{X_i\mid Z}(\xh_i;z')\\
        &= P_Z(z') && \prod_{i\in o} P_{X_i\mid Z}(x_i;z')\prod_{i\in m} P_{X_i\mid Z}(\hat{x}_i;z')\prod_{i=1}^p P_{X_i\mid Z}(\xt_i;z')\\
        &=P_{\hat{X},\Xt,Z'}(\xh,\xt,z')
\end{alignat*}
The first equality uses Eq. \ref{proof:gz2} with the swap definition applied to each factor in Eq. \ref{proof:gz2}e. The second equality follows grouping the variables. Pairwise exchangeability of $\Xh,\Xt$ follows as above statement holds for all $z'$. For continuous variables summations can be replaced with integrations.

\end{proof}
% \section{Theorem}

% \begin{equation}
% \begin{split}
%     P_{X,\Xt,Z'}(x,\xt,z')&=P_{X\mid Z}(\xt;z')\sum_{\hat{z}}P_{Z'\mid X,\hat{Z}}(z';x,\hat{z})P_{X,Z}(x,\hat{z})\\
%     &=P_{X\mid Z}(\xt;z')g_T(z',x)\\
%     &=P_{X\mid Z}(\xt;z')P_{X,Z}(x,z')\\
%     &=P_{X\mid Z}(\xt;z')P_{X\mid Z}(x;z')P_{Z}(z')\\
% \end{split}
% \end{equation}


==> chap1/miss/tex/proof_hmm.tex <==
% \clearpage
\subsection{HMM Latent Variable Posterior Sampling}
% \section{HMM Latent Variable Posterior Sampling}
% Given $x_o$, we define $o(t)\defeq o\cap\{1,\dots,t\}$. Algorithm \ref{alg:hmm_post} is an extension of the ``Forward backward sampling for a HMM'' of \cite{sesiaGeneHuntingHidden2019} to the missing data setting. In the missing data setting, multiplication with the emission probabilities $P_{X_t\mid Z_t}$ needs to be applied only if $t$ is observed. That is equivalent to setting the emission probabilities to one for missing values as discussed in
% \cite{broman2009guide} Appendix D.2. 

% \begin{algorithm}[H]
% \caption{HMM Latent Posterior Sampling with Missing Values}\label{alg:hmm_post}
% \begin{algorithmic}
% \STATE {\bfseries Input:} $x_o, P_{Z_1}, P_{X\mid Z}$,$P_{\Zt \mid Z}, o$
% \FOR{\texttt{$t=1,\dots,T$}}
%     \IF{ $t=1$}
%         \STATE $\alpha_t(z_t) \leftarrow P_{Z_1}(z_1)$
%     \ELSE 
%         \STATE $\alpha_t(z_t) \leftarrow  \sum_{z_{t-1}}P_{Z_t\mid Z_{t-1}}(z_t\mid z_{t-1})\alpha_{t-1}(z_{t-1})$
%     \ENDIF
%     \IF{$t\in o$}
%     \STATE $\alpha_t(z_t) \leftarrow \alpha_t(z_t)P_{X_t\mid Z_t}(x_t;z_t)$
%     \ENDIF
% \ENDFOR
% \FOR{\texttt{$t=T,\dots,1$}}
%     \IF{$t=T$}
%         \STATE $P_{\hat{Z}_T\mid X_{o}}(z_T;x_{o})\leftarrow\dfrac{\alpha_{t}(z_t)}{\sum_{z_t'}\alpha_{t}(z_t')}$
%         \STATE $\hat{z}_T\sim P_{\hat{Z}_T\mid X_{o}}(\cdot;x_{o})$
%     \ELSE
%         \STATE $P_{\hat{Z}_t\mid \hat{Z}_{t+1},X_{o(t)}}(z_t;z_{t+1},x_{o(t)})\leftarrow\dfrac{P_{Z_{t+1}\mid Z_t}(z_{t+1};z_t)\alpha_{t}(z_t)}{\sum_{z_t'}P_{Z_{t+1}\mid Z_t}(z_{t+1};z_t')\alpha_{t}(z_t')}$
%         \STATE $\hat{z}_t\sim P_{\hat{Z}_t\mid \hat{Z}_{t+1},X_{o(t)}}(;\hat{z}_{t+1},x_{o(t)})$
%     \ENDIF
% \ENDFOR
% \STATE {\bfseries Output:}  $\{\hat{z_t}\}_{t=1}^T$ 
% \end{algorithmic}
% \end{algorithm}
\begin{prop}\label{thm:hmm_post}
Let $\hat{Z}$ denote the output of Algorithm \ref{alg:hmm_post} with the input $X_o$, then the resulting latent posterior distribution satisfies $P_{\hat{Z}\mid X_o}(z;x_o)=P_{Z\mid X_o}(z;x_o)$.
\end{prop}


To show that Algorithm \ref{alg:hmm_post} provides valid posterior samples we first prove to two useful lemmas. Our proof is an extension of the proof of Proposition 3 in \cite{sesiaGeneHuntingHidden2019} to the setting with missing values. We denote $o\cap\{1,\dots,t\}$ as $o(t)$.

\begin{lem}\label{lem:post_hmm}

If $\alpha_t(z_t)$ is calculated as in Algorithm \ref{alg:hmm_post} then,
$\alpha_t(z_t)=P_{Z_t,X_{o(t)}}(z_t,x_{o(t)})$.
\end{lem}
\begin{proof}


Proof by induction:

Base:
% P_{Z_t,X_{o(t)}}(z_t,x_{o(t)})
\begin{subequations}\label{eq:lem_3_1}
\begin{align}
  \alpha_1(z_1)&=\begin{cases}
    P_{X_1\mid Z_1}(x_1;z_1)P_{Z_1}(z_1),&\text{if } 1\in o\\
    P_{Z_1}(z_1),  &\text{o.w.}
\end{cases}\\&=
\begin{cases}
    P_{Z_1,X_1}(z_1,x_1),&\text{if } 1\in o\\
    P_{Z_1}(z_1),  &\text{o.w.}
\end{cases}\\
&=P_{Z_t,X_{o(1)}}(z_1,x_{o(1)})
\end{align}
\end{subequations}

\ref{eq:lem_3_1}a follows from Algorithm \ref{alg:hmm_post}. \ref{eq:lem_3_1}b uses the definition of conditional indepedence. \ref{eq:lem_3_1}c uses the definition of $x_{o(1)}$.

Induction step k:

\begin{subequations}\label{eq:lem_3_2}
\begin{align}
\gamma_{k}(z_k)&\defeq \sum_{z_{k-1}}P_{Z_k\mid Z_{k-1}}(z_k; z_{k-1})\alpha_{k-1}(z_{k-1})\\
&=\sum_{z_{k-1}}P_{Z_k\mid Z_{k-1}}(z_k; z_{k-1})P_{Z_{k-1},X_{o(k-1)}}(z_{k-1},x_{o(k-1)})\\
&=\sum_{z_{k-1}}P_{Z_k\mid Z_{k-1},X_{o(k-1)}}(z_k; z_{k-1},x_{o(k-1)})P_{Z_{k-1},X_{o(k-1)}}(z_{k-1},x_{o(k-1)})\\
&=\sum_{z_{k-1}}P_{Z_k, Z_{k-1},X_{o(k-1)}}(z_k, z_{k-1},x_{o(k-1)})\\
&=P_{Z_k,X_{o(k-1)}}(z_k,x_{o(k-1)})
\end{align}
\end{subequations}

\ref{eq:lem_3_2}b follows from the induction assumption at step $k-1$. \ref{eq:lem_3_2}c uses the conditional independence of the HMM. \ref{eq:lem_3_2}d uses the definition of conditional independence. \ref{eq:lem_3_2}e uses the law of total probability.

If $k\in o$, then 
\begin{subequations}\label{eq:lem_3_3}
\begin{align}
\alpha_k(z_k)&=P_{X_k\mid Z_k}(x_k;z_k)\gamma_{k}(z_k)\\
&=P_{X_k\mid Z_k,X_{o(k-1)}}(x_k;z_k,x_{o(k-1)})\gamma_{k}(z_k)\\
&=P_{X_k\mid Z_k,X_{o(k-1)}}(x_k;z_k,x_{o(k-1)})P_{Z_k,X_{o(k-1)}}(z_k,x_{o(k-1)})\\
&=P_{X_k, Z_k,X_{o(k-1)}}(x_k,z_k,x_{o(k-1)})\\
&=P_{Z_k,X_{o(k)}}(z_k,x_{o(k)})
% &=P_{Z_k,X_{o(k-1)}}(z_k,x_{o(k-1)})\\
% &=P_{Z_k,X_{o(k)}}(z_k,x_{o(k)})
\end{align}
\end{subequations}

\ref{eq:lem_3_3}a follows from Algorithm \ref{alg:hmm_post}. \ref{eq:lem_3_3}b follows from the conditional independence of HMM. \ref{eq:lem_3_3}c follows from Eq. \ref{eq:lem_3_2}. \ref{eq:lem_3_3}d follows from definition of conditional probability.

If $k\not\in o$, then 
\begin{subequations}\label{eq:lem_3_4}
\begin{align}
\alpha_k(z_k)&=\gamma_{k}(z_k)\\
&=P_{Z_k,X_{o(k-1)}}(z_k,x_{o(k-1)})\\
&=P_{Z_k,X_{o(k)}}(z_k,x_{o(k)})
\end{align}
\end{subequations}

\ref{eq:lem_3_4}a follows from Algorithm \ref{alg:hmm_post} as $k\not \in o$. \ref{eq:lem_3_4}b follows from Eq. \ref{eq:lem_3_2}. \ref{eq:lem_3_4}c follows from definition of $o(k)$.

\end{proof}

\begin{lem}\label{lem:post_hmm2}
% If $\alpha_t(z_t)$ is calculated as in Algorithm \ref{alg:hmm_post} then,
Let $P_{\hat{Z}_T\mid X_o}$ and $P_{\hat{Z}_t\mid \hat{Z}_{t+1},X_{o(t)}}$ denote the probabilities computed in Algorithm \ref{alg:hmm_post} then
${P_{\hat{Z}_t\mid \hat{Z}_{t+1},X_{o(t)}}(z_t; z_{t+1},x_{o(t)})=P_{Z_t\mid Z_{t+1},X_{o(t)}}(z_t; z_{t+1},x_{o(t)})}$ and ${P_{\hat{Z}_T\mid X_o}(z_T; x_o)=P_{Z_T\mid X_o}(z_T; x_o)}$
% \[P_{Z_t\mid Z_{t+1},X_{o(t)}}(z_t;z_{t+1},x_{o(t)})=\dfrac{P_{Z_{t+1}\mid Z_t}(z_{t+1};z_t)\alpha_{t}(z_t)}{\sum_{z_t'}P_{Z_{t+1}\mid Z_t}(z_{t+1};z_t')\alpha_{t}(z_t')}\]
\end{lem}
\begin{proof}

\begin{subequations}
\begin{align}
        P_{Z_t\mid Z_{t+1},X_{o(t)}}(z_t;z_{t+1},x_{o(t)})&=\dfrac{P_{Z_t,Z_{t+1},X_{o(t)}}(z_t,z_{t+1},x_{o(t)})}{P_{Z_{t+1},X_{o(t)}}(z_{t+1},x_{o(t)})}\\
        &=\dfrac{P_{Z_{t+1}\mid Z_t}(z_{t+1};z_t)\alpha_{t}(z_t)}{\sum_{z_t'}P_{Z_{t+1}\mid Z_t}(z_{t+1};z_t')\alpha_{t}(z_t')}\\
        &=P_{\hat{Z}_t\mid \hat{Z}_{t+1},X_{o(t)}}(z_t;z_{t+1},x_{o(t)})
\end{align}
\end{subequations}
The first line follows from the definition of conditional probability. The second line uses chain rule, conditional independence of the HMM and $\alpha_{t}(z_t)=P_{Z_t,X_{o(t)}}(z_t,x_{o(t)})$ from Lemma \ref{lem:post_hmm}. The last equality follows from Algorithm \ref{alg:hmm_post}. Similarly, at $t=T$
\begin{subequations}
\begin{align}
        P_{Z_T\mid X_o}(z_T;x_o)&= \dfrac{P_{Z_T,X_o}(z_T,x_o)}{P_{X_o}(x_o)}\\
        &=\dfrac{\alpha_T(z_T)}{\sum_{z_T'}\alpha_T(z_T')}\\
        &=P_{\hat{Z}_T\mid X_o}(z_T;x_o)
\end{align}
\end{subequations}

The first line follows from definition of conditional probability. The second line from Lemma \ref{lem:post_hmm}. The third line follows from Algorithm \ref{alg:hmm_post}.
\end{proof}
% To proove the above statement we prove Lemmas

% let $\alpha_t(z_t)\defeq P_{Z_t,X_{o(t)}}(z_t,x_{o(t)})$. Assume $t\in o$, then
\begin{proof}[Proof of Proposition \ref{thm:hmm_post}]

The resulting $P_{\hat{Z}\mid X_o}$ from Algorithm \ref{alg:hmm_post} can be factored using the sampling structure as follows:

\begin{subequations}\label{eq:prop_2}
\begin{align}
        P_{\hat{Z}\mid X_o}(\hat{z};x_o)
        &=P_{\hat{Z}_T\mid X_o}(\hat{z}_T;x_o)\prod_{t=1}^{T-1}P_{\hat{Z_t}\mid \hat{Z}_{t+1:T},X_o}(\hat{z_t};  \hat{z}_{t+1:T}, x_o)\\
        &=P_{\hat{Z}_T\mid X_o}(\hat{z}_T;x_o)\prod_{t=1}^{T-1}P_{\hat{Z_t}\mid \hat{Z}_{t+1}, X_{o(t)}}(\hat{z_t}; \hat{z}_{t+1}, x_{o(t)})\\
        &=P_{Z_T\mid X_o}(\hat{z}_T;x_o)\prod_{t=1}^{T-1} P_{Z_t\mid Z_{t+1},X_{o(t)}}(\zh_t; \zh_{t+1},x_{o(t)})\\
        &=P_{Z_T\mid X_o}(\zh_T;x_o)\prod_{t=1}^{T-1} P_{Z_t\mid Z_{t+1:T},X_o}(\zh_t;\zh_{t+1:T},x_o)\\
        &=P_{Z\mid X_o}(\hat{z};x_o)
\end{align}
\end{subequations}


\ref{eq:prop_2}a uses the chain rule. \ref{eq:prop_2}b uses the conditional independence following from the sampling order. \ref{eq:prop_2}c follows from Lemma \ref{lem:post_hmm2}. \ref{eq:prop_2}d follows from applying d-separation to the HMM graph. \ref{eq:prop_2}e again uses the chain rule. 
\end{proof}


==> chap1/miss/tex/proof_lami.tex <==
\begin{definition}
$P_{Z',\Xt\mid \Zh}(z',\xt;\zh)$ is a 
\end{definition}
\begin{thm}
Let $P_{Z',\Xt\mid \Zh}(z',\xt;\zh)$ denote a probability density s.t. when $\Zh\sim P_{Z\mid X}(;X)$ and $(Z',\Xt) \sim P_{Z',\Xt\mid \Zh}(;\Zh)$ then $X,\Xt$ becomes pairwise exchangeable. If only the observed variables are used i.e. $\Zh'\sim P_{Z\mid X_o}(;X_o)$, $\Xh_m\sim P_{X_m\mid Z}(;\Zh')$, and $(Z'',\Xt') \sim P_{Z',\Xt\mid \Zh}(;\Zh')$. Then let $\Xh=(\Xh_1,\dots,\Xh_p)^T$ denote the imputed vector where $\Xh_o=X_o$ then $\Xh,\Xt'$ will be pairwise exchangeable.

\end{thm}

==> chap1/miss/tex/proof_latent.tex <==
\subsection{Proof of Theorem \ref{thm:latent}}\label{app:latent}

\begin{proof}[Proof of Theorem \ref{thm:latent}]

The theorem assumes when the joint distribution of the observations and posterior sample $P_{X,\Zh}$ equals to $P_{X,Z}$, sampling procedure results in \pe $X, \Xt$. Therefore, it's sufficient to show the joint distribution of the imputed observation vector and the posterior sample maintains the distribution $P_{X,Z}$. Formally, we need to show ${P_{\Xh,\Zh}(\xh, \zh)=P_{X,Z}(\xh, \zh)}$ holds. 

We first start with ${\zh \in \mathcal{Z}}$, $ {\xh\in \mathcal{X}}$ s.t. $P_{X_o,Z}(\xh_o,\zh)>0$ where $\mathcal{Z}$ and $\mathcal{X}$ are the domains of $P_{Z}$ and $P_{X}$ (respt.). Let ${\mathcal{R}\defeq \{r\in \{0,1\}^p:P_{X_o,R}(\xh_o,r)>0\}}$

\begin{subequations}\label{proof:theo_3}
\begin{align}
        P_{\Xh,\Zh}(\xh, \zh)&=\sum_{r\in \{0,1\}^p} P_{\Xh,\Zh\mid R}(\xh, \zh;r)P_{R}(r)\\
        &=\sum_{r\in \{0,1\}^p} P_{\Xh_m\mid\Zh,R}(\xh_m; \zh,r)P_{\Zh \mid \Xh_o, R}(\zh ; \xh_o, r)P_{\Xh_o \mid R}(\xh_o; r)P_{R}(r)\\
        &=\sum_{r\in \{0,1\}^p} P_{X_m\mid Z}(\xh_m; \zh)P_{Z \mid X_o}(\zh ; \xh_o)P_{X_o \mid R}(\xh_o; r)P_{R}(r)\\
        %check zero division?
        &=\sum_{r\in \{0,1\}^p} P_{X_m\mid Z, X_o}(\xh_m; \zh,\xh_o)P_{Z \mid X_o}(\zh ; \xh_o)P_{X_o \mid R}(\xh_o; r)P_{R}(r)\\
        &=\sum_{r\in \{0,1\}^p} P_{X_m, Z\mid X_o}(\xh_m, \zh;\xh_o)P_{X_o \mid R}(\xh_o; r)P_{R}(r)\\
        &=\sum_{r\in \{0,1\}^p} P_{Z\mid X_m, X_o}( \zh;\xh_m,\xh_o)P_{X_m\mid X_o}(\xh_m;\xh_o)P_{X_o \mid R}(\xh_o; r)P_{R}(r)\\
        &=\sum_{\forall r \in \mathcal{R}} P_{Z\mid X}( \zh;\xh)P_{X_m\mid X_o}(\xh_m;\xh_o)P_{X_o \mid R}(\xh_o; r)P_{R}(r)\\
        &=\sum_{\forall r \in \mathcal{R}} P_{Z\mid X}( \zh;\xh)P_{X_m\mid X_o,R}(\xh_m;\xh_o,r)P_{X_o \mid R}(\xh_o; r)P_{R}(r)\\
        &=P_{Z\mid X}( \zh;\xh) \sum_{\forall r \in \mathcal{R}} P_{X_m, X_o\mid R}(\xh_m,\xh_o; r)P_{R}(r)\\
        &=P_{Z\mid X}( \zh;\xh) \sum_{\forall r \in \mathcal{R}} P_{X\mid R}(\xh; r)P_{R}(r)\\
        &=P_{Z\mid X}( \zh;\xh) P_{X}(\xh)\\
        &=P_{X,Z}(\xh,\zh)
        % P_{\hat{Z}_t\mid \hat{Z}_{t+1},X_{o(t)}}(z_t;z_{t+1},x_{o(t)})
\end{align}
\end{subequations}
\ref{proof:theo_3}a uses the total law of probability. \ref{proof:theo_3}b uses the chain rule and conditional independence resulting from the order the random vectors are sampled. \ref{proof:theo_3}c uses both $\Xh_o=X_o$ and the conditional distributions used to sample $\Xh_m$ and $\Zh$. \ref{proof:theo_3}d uses $X_m \indep X_o \mid Z$ and $P_{X_o\mid Z}(\xh_o;\zh)>0$. \ref{proof:theo_3}e follows from chain rule. \ref{proof:theo_3}f uses chain rule. \ref{proof:theo_3}g uses $\{1,\dots,p\}=m\cup o$, and for all $r\notin \mathcal{R}$ the inner summation terms are equal to zero i.e. $P_{X_o\mid R}(\xh_o;r)=0$. \ref{proof:theo_3}h uses MAR (or MCAR) assumption i.e. $X_m\indep R \mid X_o $ and $P_{X_o,R}(\xh_o,r)>0$. Using the equality $P_{X_m\mid X_o}=P_{X_m\mid X_o, R}$ was inspired by the Example 2 of Section 3.1.1.  \cite{mohanGraphicalModelsInference2017}. \ref{proof:theo_3}i uses distributive property and chain rule. \ref{proof:theo_3}j again uses $\{1,\dots,p\}=m\cup o$. \ref{proof:theo_3}k follows from the total low of probability and for all $r\notin \mathcal{R}$, $P_{X,R}(\xh,r)=0$. \ref{proof:theo_3}l uses the definition of conditional probability.

We now turn our attention to the remaining variables ${\zh \in \mathcal{Z}}$, $ {\xh\in \mathcal{X}}$ s.t.  $P_{X_o,Z}(\xh_o,\zh)=0$. Then, $P_{X,Z}(\xh,\zh)=0$ and $P_{Z\mid X_o}(\zh;\xh_o)=0$ also holds. From \ref{proof:theo_3}c 

\begin{equation*}
    \begin{split}
        P_{\Xh,\Zh}(\xh, \zh)&=\sum_{r\in \{0,1\}^p} P_{X_m\mid Z}(\xh_m; \zh)P_{Z \mid X_o}(\zh ; \xh_o)P_{X_o \mid R}(\xh_o; r)P_{R}(r)\\
        &=0\\
        &=P_{X,Z}(\xh,\zh)
    \end{split}
\end{equation*}
\end{proof}
% P_{\Xh,\Zh}(\xh, \zh)

==> chap1/miss/tex/proof_mar.tex <==
\subsection{Proof of Lemma \ref{lem:mar}}\label{app:mar}
\begin{proof}[Proof of Lemma \ref{lem:mar}]

We first prove it for MCAR setting. Let $\mathcal{R}\defeq \{r\in \{0,1\}^p:P_{\Xh,R}(\xh,r)>0\}$, $\forall \ \xh$
\begin{subequations}\label{proof:mar}
\begin{align}
% \begin{equation}
% \begin{split}
    P_{\hat{X}}(\hat{x})&=\sum_{\forall r \in \mathcal{R}}P_{\Xh\mid R}(\xh;r)P_R(r)\\
    %
    &=\sum_{\forall r \in \mathcal{R}}P_{\Xh_m\mid \Xh_o, R}(\xh_m;\xh_o,r)P_{\Xh_o\mid R}(\xh_o;r)P_R(r)\\
    %
    &=\sum_{\forall r \in \mathcal{R}}P_{\Xh_m\mid \Xh_o, R}(\xh_m;\xh_o,r)P_{X_o\mid R}(\xh_o;r)P_R(r)\\
    %
    &=\sum_{\forall r \in \mathcal{R}}P_{X_m\mid X_o}(\xh_m;\xh_o)P_{X_o}(\xh_o)P_R(r)\\
    %
    &=P_{X_m\mid X_o}(\xh_m;\xh_o)P_{X_o}(\xh_o)\\
    %
    &=P_{X}(\xh)\\
\end{align}
\end{subequations}
% \end{split}
% \end{equation}

\ref{proof:mar}a follows from law of total probability and chain rule. \ref{proof:mar}b follows from $m=\{i:R_i=1\}$ and $o=\{i:R_i=0\}$. \ref{proof:mar}c uses $\hat{X}_o=X_o$. \ref{proof:mar}d follows from posterior sampling and MCAR i.e. $X\indep R$. We next proceed with the more general MAR setting. $\forall \ \xh$

\begin{subequations}\label{proof:mcar}
\begin{align}
    % P_{\hat{X}}(\hat{x})&=\sum_{r}P_{\Xh\mid R}(\xh;r)P_R(r)\\
    %
    % &=\sum_{r}P_{\Xh_m\mid \Xh_o, R}(\xh_m;\xh_o,r)P_{\Xh_o\mid R}(\xh_o;r)P_R(r)\\
    %
    % &=\sum_{r}P_{\Xh_m\mid \Xh_o, R}(\xh_m;\xh_o,r)P_{X_o\mid R}(\xh_o;r)P_R(r)\\
    %
    P_{\hat{X}}(\hat{x})&=\sum_{\forall r \in \mathcal{R}}P_{X_m\mid X_o}(\xh_m;\xh_o)P_{X_o\mid R}(\xh_o;r)P_R(r)\\
    %
    &=\sum_{\forall r \in \mathcal{R}}P_{X_m\mid X_o, R}(\xh_m;\xh_o,r)P_{X_o\mid R}(\xh_o;r)P_R(r)\\
    %
    &=\sum_{\forall r \in \mathcal{R}}P_{X, R}(\xh,r)\\
    &=P_{X}(\xh)\\
\end{align}
\end{subequations}

\ref{proof:mcar}a follows from the posterior sampling. \ref{proof:mcar}b follows from MAR assumption i.e. $X_m\indep R \mid X_o $ and $P_{X_o,R}(x_o,r)>0$. $r\in \mathcal{R}$ implies $P_{\Xh_o,R}(\xh_o,r)>0$ which implies $P_{X_o,R}(x_o,r)>0$. The $P_{X_m\mid X_o}=P_{X_m\mid X_o, R}$ property was inspired by the Example 2 of Section 3.1.1.  \cite{mohanGraphicalModelsInference2017}.


\end{proof}

==> chap1/miss/tex/proof_mb.tex <==
\section{MB and Conditionally Pairwise Equivalence}
We denote $X$ as a $p$-dimensional random vector, $Y$ a R.V., $X_j$ j'th R.V of $X$, and $X_{-j}=\{X_l:l\neq j\}$. Given set $M$, $X_M=\{X_l:l\in M\}$ denotes the corresp. R.Vs and the complement of $M$ is denoted by  $M'=\{1,\dots,p\}\setminus M$.  

\begin{definition}
Let $M\subseteq\{1,\dots,p\}$. $X_M$ is the Markov Blanket (MB) of $Y$ if it's the smallest subset such that 

\[Y\indep X_{M'} \mid X_M\]

\end{definition}

\begin{thm}\label{thm:mb}
Let $X,Y$ denote two random vector and $X_M$ denote the MB of $Y$. Given $P_{X,Y}(x,y)>0 \ \forall x,y$, $Y\nindep X_i \mid X_{-i}$ holds iff $i\in M$.
\end{thm}
\begin{proof}

We start with the direction $Y\nindep X_i \mid X_{-i}$ $\Rightarrow$ $i\in M$. Proof by contradiction, assume $i\in M$ and $Y\indep X_i \mid X_{-i}$. Then, $\forall x,y$

% \begin{equation}\label{eq2}
% \begin{split}
\begin{subequations}\label{eq2}
\begin{align}
    P_{Y\mid X_{-i}}(y;x_{-i})&=P_{Y\mid X}(y;x)\\
        P_{Y\mid X_{-i}}(y;x_{-i})&=P_{Y\mid X_M}(y;x_M)\\
    \dfrac{P_{Y,X_{-i}}(y,x_{-i})}{P_{X_{-i}}(x_{-i})}&=P_{Y\mid X_M}(y;x_M)\\
    P_{Y,X_{-i}}(y,x_{-i})&=P_{Y\mid X_M}(y;x_M)P_{X_{-i}}(x_{-i})\\
    \sum_{x_{M'}}P_{Y,X_{-i}}(y,x_{-i})&=\sum_{x_{M'}}P_{Y\mid X_M}(y;x_M)P_{X_{-i}}(x_{-i})\\
    \sum_{x_{M'}}P_{Y,X_{M'},X_{M\setminus\{i\}}}(y,x_{M'},x_{M\setminus\{i\}})&=P_{Y\mid X_M}(y;x_M)\sum_{x_{M'}}P_{X_{M'},X_{M\setminus\{i\}}}(x_{M'},x_{M\setminus\{i\}})\\
    P_{Y,X_{M\setminus\{i\}}}(y,x_{M\setminus\{i\}})&=P_{Y\mid X_M}(y;x_M)P_{X_{M\setminus\{i\}}}(x_{M\setminus\{i\}})\\
    P_{Y\mid X_{M\setminus\{i\}}}(y\mid x_{M\setminus\{i\}})&=P_{Y\mid X_M}(y;x_M)\\
    &=P_{Y\mid X}(y;x)
\end{align}
\end{subequations}

The explanation of the properties used in each line of Eq. \ref{eq2}:
\begin{enumerate}[label=(\alph*)]
    \item $Y\indep X_i \mid X_{-i}$
    \item Definition of Markov Blanket
    \item Definition of conditional probability 
    \item Strict positivity 
    \item Both sides summed 
    \item Constant outside the summation, splitting the variables using $i\in M$ 
    \item Total law of probability \item Definition of conditional probability 
    \item Definition of Markov Blanket
\end{enumerate}


Eq. \ref{eq2} implies $Y \indep X_{(M\setminus \{i\})'}\mid X_{M\setminus \{i\}}$ which contradicts the assumption that $M$ is the MB of Y since cardinality of $M\setminus \{i\}$ is one less than of $M$. Note if we use  integration instead of the summation the proof can be used for the continuous R.Vs. An alternative proof for the discrete R.Vs can be done using the Intersection condition in \cite{10.5555/534975}.
% \begin{equation}\label{eq2}
%   \begin{split}
%       Y&\indep X_{M'} \mid X_{M\setminus\{i\}}, X_i\\
%       Y&\indep X_i \mid X_{M\setminus\{i\}}, X_{M'}\\
%       \Rightarrow Y&\indep X_{M'}, X_i \mid X_{M\setminus\{i\}}\\\
%   \end{split} 
% \end{equation}

% The first and second statements follows from definition of $MB$ and $Y\indep X_i \mid X_{-i}$ respectively. The implication follows from the Lemma \ref{lem4}. Furthermore, the final statement implies $X_{M \setminus \{i\}}$ is the MB of a Y because
% $M'\cup \{i\} \cup (M \setminus \{i\})=\{1,\dots,p\}$. That contradicts the assumption that $X_M$ is the MB of Y since cardinality of the set $M\setminus \{i\}$ is one less than of $M$.

\vspace{1cm}

We next proceed to proving the second direction $i\in M$ $\Rightarrow$ $Y\nindep X_i \mid X_{-i}$. We use proof by contradiction and assume $i\notin M$.
\begin{equation}\label{eq:mb}
    \begin{split}
        &Y \indep X_{M'} \mid X_M\\
        \Rightarrow \ &Y \indep X_{M'\setminus \{i\}} \mid X_M\\
        \Rightarrow &P_{Y\mid X_{-i}}(y;x_{-i})=P_{Y\mid X_{M}}(y;x_{M}), \ \forall x,y
    \end{split}
\end{equation}
The first implication follows from marginalizing $X_i$. The next one follows from the strict positiveness and $x_{M\cup M'\setminus \{i\}}=x_{-i}$.

\end{proof}
% \begin{lem}
% Let $X_M$ denote the MB of $Y$. Given $P_{X,Y}(x,y)>0 \ \forall x,y$, if $Y\nindep X_i \mid X_{-i}$ then $i\in M$.
% \end{lem}
% \begin{proof}
% This direction is much simpler.
% \end{proof}

==> chap1/miss/tex/proof_sesia.tex <==
\subsection{Theorem \ref{thm:sesia}}\label{app:sesia}

We first prove a useful Lemma.
\begin{lem}\label{lem:p_z_x}
Given random vectors $X_m, X_o,Z$, let $\Zh\sim P_{Z\mid X_o}(\cdot;X_o)$ and $\Xh_m\sim P_{X_m\mid Z}(\cdot;\Zh)$. If $X_m\indep X_o \mid Z$, then $P_{\Xh_m\mid X_o}(\xh_m; x_o)=P_{X_m\mid X_o}(\xh_m; x_o)$ holds for all $\xh_m,x_o$.
\end{lem}
\begin{proof}[Proof of Lemma \ref{lem:p_z_x}]
Let $\mathcal{Z}\defeq\{z: P_{\Xh_m,\Zh\mid X_o}(\xh_m,\zh; x_o)>0\}$

\begin{subequations}\label{proof:p_z_x}
\begin{align}
        P_{\Xh_m\mid X_o}(\xh_m; x_o)&=\sum_{\zh\in\mathcal{Z}}P_{\Xh_m,\Zh \mid X_o}(\xh_m,\zh; x_o)\\
        &=\sum_{\zh\in\mathcal{Z}}P_{\Xh_m \mid \Zh, X_o}(\xh_m; \zh, x_o)P_{ \Zh \mid X_o}(\zh; x_o)\\
        &=\sum_{\zh\in\mathcal{Z}}P_{\Xh_m \mid \Zh}(\xh_m; \zh)P_{ Z \mid X_o}(\zh; x_o)\\
        &=\sum_{\zh\in\mathcal{Z}}P_{X_m \mid Z}(\xh_m; \zh)P_{ Z \mid X_o}(\zh; x_o)\\
        &=\sum_{\zh\in\mathcal{Z}}P_{X_m\mid Z, X_o}(\xh_m; \zh, x_o)P_{ Z \mid X_o}(\zh; x_o)\\
        &=\sum_{\zh\in\mathcal{Z}}P_{X_m, Z\mid X_o}(\xh_m\zh; x_o)\\
        &=P_{X_m \mid X_o}(\xh_m; x_o)\\
\end{align}
\end{subequations}

The equality $P_{X_m \mid Z}=P_{X_m\mid Z, X_o}$ used in \ref{proof:p_z_x}e follows from  $X_m\indep X_o \mid Z$ and $z\in \mathcal{Z}$. Because $z\in \mathcal{Z}$ implies $P_{\Zh,X_o}(\zh,x_o)>0$ which then implies $P_{Z,X_o}(\zh,x_o)>0$.
\end{proof}
\begin{proof}[Proof of Theorem \ref{thm:sesia}]

Algorithm \ref{alg:sesia}, uses $\Zh\sim P_{Z\mid X_o}(\cdot;X_o)$ and $\Xh_m\sim P_{X_m\mid Z}(\cdot;\Zh)$. Therefore, from Lemma \ref{lem:p_z_x}, we have $P_{\Xh_m\mid X_o}(\xh_m; x_o)=P_{X_m\mid X_o}(\xh_m; x_o)$ for all $\xh_m,x_o$. Then, combining that with Lemma \ref{lem:mar} results in $P_X=P_{\Xh}$ as MAR or MCAR holds. 

\begin{subequations}\label{proof:sesia}
\begin{align}
        P_{\hat{X},\Xt,\Zh,Z'}(\xh,\xt,\zh,z')
        &=P_{\Xt_o\mid Z'}(\xt_o; z')P_{\Xt_m\mid Z'}(\xt_m; z')P_{Z'\mid \hat{Z}}(z';\hat{z})P_{\Xh_m\mid \Zh}P_{X_o\mid \Zh}(x_o; \zh)P_{\Zh}(\hat{z})\\
        &=P_{X_o\mid Z}(\xt_o; z')P_{X_m\mid Z}(\xt_m; z')P_{X_o\mid Z}(x_o; \zh)P_{X_m\mid Z}(\xh_m; \zh)P_{Z',\hat{Z}}(z',\hat{z})\\
        &=P_{Z',\hat{Z}}(z',\hat{z})\prod_{i\in o}P_{X_i\mid Z_i}(x_i;\zh_i)\prod_{i\in m}P_{X_i\mid Z_i}(\xh_i;\zh_i)\prod_{i=1}^p P_{X_i\mid Z_i}(\xt_i;z_i')
\end{align}
\end{subequations}

% In an HMM

\begin{alignat*}{3}
 \hspace*{-2cm}
        P_{\hat{X},\Xt,\Zh,Z'}((\xh,\xt)_\swap,(\zh,z')_\swap)&=P_{Z',\hat{Z}}((z',\hat{z})_\swap)&&
        \prod_{i\in o\setminus S}P_{X_i\mid Z_i}(x_i;\zh_i)\prod_{i\in o\cap S}P_{X_i\mid Z_i}(\xt_i;z_i')\\
        & &&\prod_{i\in m\setminus S}P_{X_i\mid Z_i}(\xh_i;\zh_i)
        \prod_{i\in m\cap S}P_{X_i\mid Z_i}(\xt_i;z_i')\\
        & &&\prod_{i\in o\setminus S}P_{X_i\mid Z_i}(\xt_i;z_i')\prod_{i\in o\cap S}P_{X_i\mid Z_i}(x_i;\zh_i)
        \\
        & && \prod_{i\in m\setminus S}P_{X_i\mid Z_i}(\xt_i;z_i')
        \prod_{i\in m\cap S}P_{X_i\mid Z_i}(\xh_i;\zh_i)\\
        & =P_{Z',\hat{Z}}(z',\hat{z})&&\prod_{i\in o}P_{X_i\mid Z_i}(x_i;\zh_i)\prod_{i\in m}P_{X_i\mid Z_i}(\xh_i;\zh_i)\prod_{i=1}^p P_{X_i\mid Z_i}(\xt_i;z_i')\\
        &= P_{\hat{X},\Xt,\Zh,Z'}(\xh,\xt,\zh,z')
\end{alignat*}


$P_{Z',\hat{Z}}((z',\hat{z})_\swap)=P_{Z',\hat{Z}}(z',\hat{z})$ follows from $P_{\Zt \mid Z}$ is pairwise exchangeable with respect to $P_Z$.
\end{proof}

%     \end{split}
% \end{equation}


% \begin{equation}
%     \begin{split}
%         &\zh \sim P_{Z\mid X_o}(\cdot;x_o)\\
%         &\xh_m \sim P_{X_m\mid Z}(\cdot;\zh)\\
%         &z' \sim \text{SCIP}(\zh)\\
%         &\xt_m \sim P_{X_m\mid Z}(\cdot;z')\\
%         &\xt_o \sim P_{X_o\mid Z}(\cdot;z')
%     \end{split}
% \end{equation}

% \begin{equation}
%     \begin{split}
%         P_{\hat{X},\Xt,\Zh,Z'}(\xh,\xt,\zh,z')
%         &=P_{\Xt_o\mid Z'}(\xt_o; z')P_{\Xt_m\mid Z'}(\xt_m; z')P_{Z'\mid \hat{Z}}(z';\hat{z})P_{\Xh_m\mid \Zh}P_{X_o\mid \Zh}(x_o; \zh)P_{\Zh}(\hat{z})\\
%         &=P_{X_o\mid Z}(\xt_o; z')P_{X_m\mid Z}(\xt_m; z')P_{X_o\mid Z}(x_o; \zh)P_{X_m\mid Z}(\xh_m; \zh)P_{Z',\hat{Z}}(z',\hat{z})\\
%     \end{split}    
% \end{equation}
% \begin{equation}
% \begin{split}
%     P_{\hat{X},\Xt,\Zh,Z'}(\xh,\xt,\zh,z')&=P_{Z',\hat{Z}}(z',\hat{z})\prod_{i\in o}P_{X_i\mid Z_i}(x_i;\zh_i)\prod_{i\in m}P_{X_i\mid Z_i}(\xh_i;\zh_i)\prod_{i=1}^p P_{X_i\mid Z_i}(\xt_i;z_i')
%     % \prod_{i\in m}P_{X_i\mid Z_i}(\xt_i;z_i')
% \end{split}
% \end{equation}

==> chap1/miss/tex/proof_uni.tex <==
\subsection{Theorem \ref{thm:uni}}\label{app:uni}

\textbf{Correction:} In the submitted manuscript, we have denoted that \pe of Theorem \ref{thm:uni} holds for both MAR and MCAR. We're weren't able to prove the statement under MAR and decided to restrict the theorem to the MCAR setting. The revised Theorem \ref{thm:uni} is given below:

\newtheorem*{thm*}{Theorem}

\begin{thm*}\label{thm:corrected}

Let $\Xh=(\Xh_1,\dots,\Xh_p)^T$ denote the imputed vector where $\Xh_o=X_o$ and ${\hat{X}_{m_j}\sim P_{X_{m_j}}(\cdot) \ j=1,\dots, |m|}$. We assume $P_{X,R}$ satisfies MCAR. If $\Xt_o \sim P_{\Xt_o\mid X_o}(\cdot;\hat{X_o})$, $P_{\Xt_o\mid X_o}$ is pairwise exchangeable with respect to $P_{X_o}$, and $\Xt_{m_j}\sim P_{X_{m_j}}(\cdot) \ j=1,\dots, |m|$ then $\hat{X}$ and $\Xt$ are pairwise exchangeable.
\end{thm*}

To prove Theorem \ref{thm:corrected} we first show a useful lemma regarding the \pety of fully factored joint distributions.

\begin{lem}\label{lem:factor}
If ${\displaystyle P_X(x)=\prod_{j=1}^{p} P_{X_j}(x_j)}$ and $P_{\Xt}(x)=P_X(x)$, then $X,\Xt$ are \pe.
\end{lem}
\begin{proof}
Following Prop. 3.5.  of \cite{candesPanningGoldModelX2017}, $X,\Xt$ are \pe iff for all index $j\in\{1,\dots,p\}$, 

\begin{equation}\label{eq:iff}
    P_{X_j,\Xt_j,X_{-j},\Xt_{-j}}(x_j,\xt_j,x_{-j},\xt_{-j})=P_{X_j,\Xt_j,X_{-j},\Xt_{-j}}(\xt_j,x_j,x_{-j},\xt_{-j})
\end{equation}

We now show when $P_X$ fully factors Eq. \ref{eq:iff} holds.
% \begin{subequations}\label{proof:uni}
% \begin{align}
\begin{equation}
    \begin{split}
        P_{X_j,\Xt_j,X_{-j},\Xt_{-j}}(x_j,\xt_j,x_{-j},\xt_{-j})&=P_{X_j}(x_j)P_{X_j}(\xt_j)\prod_{l\neq j}P_{X_l}(x_l)P_{X_l}(\xt_l)\\
        &=P_{X_j}(\xt_j)P_{X_j}(x_j)\prod_{l\neq j}P_{X_l}(x_l)P_{X_l}(\xt_l)\\
        &=P_{X_j,\Xt_j,X_{-j},\Xt_{-j}}(\xt_j,x_j,x_{-j},\xt_{-j})
        % &=P_{X_o,X_m}(x_o,\hat{x}_m)
\end{split}
\end{equation}

% \begineq
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:uni}]
% Let $x=(x_o,x_m)^T$,

For all missing data masks $ r\in \{0,1\}^{p}$, because the missing values are sampled from an univariate distribution, the distribution $P_{\Xh_m,\Xt_m\mid R}(\xh_m,\xt_m;r)$ fully factors out i.e.
\[
        P_{\Xh_m,\Xt_m\mid R}(\xh_m,\xt_m;r)=\prod_{j\in m}P_{X_j}(x_j)P_{X_j}(\xt_j)
\]

where $m=\{j:r_j=1\}$ and $o=\{1,\dots,p\}\setminus m$. Therefore, from Lemma \ref{lem:factor}, $\Xh_m,\Xt_m$ are \pe conditioned on $R=r$.

Next, we show the conditional joint distribution of observed variables remains intact under MCAR.


\begin{subequations}\label{eq:uni_o}
\begin{align}
        P_{\Xt_o,\Xh_o\mid R}(\xt_o,\xh_o;r)&=P_{\Xt_o\mid \Xh_o, R}(\xt_o;\xh_o,r)P_{ \Xh_o\mid R}(\xh_o;r)\\
        &=P_{\Xt_o\mid X_o}(\xt_o;\xh_o)P_{ X_o\mid R}(\xh_o;r)\\
        &=P_{\Xt_o\mid X_o}(\xt_o;\xh_o)P_{ X_o}(\xh_o)\\
        &=P_{\Xt_o, X_o}(\xt_o,\xh_o)
\end{align}
\end{subequations}

\ref{eq:uni_o}b follows from sampling distribution $P_{\Xt_o\mid X_o}$ and $\Xh_o=X_o$. \ref{eq:uni_o}c uses the MCAR assumption. Because $ P_{\Xt_o,\Xh_o\mid R}(\xt_o,\xh_o;r)=P_{\Xt_o, X_o}(\xt_o,\xh_o)$ and $P_{\Xt_o\mid X_o}$ is \pe with respect to $P_{X_o}$ conditioned on $R=r$, $\Xh_o,\Xt_o$ are \pe.

We next use the two conditional \pety statements to show the unconditional \pety of $\hat{X}$ and $\Xt$. For any set $S\subseteq\{1,\dots,p\}$, 

\begin{subequations}\label{proof:uni}
\begin{align}
        &P_{\hat{X},\Xt}((\hat{x},\xt)_\swap)\\
        &=\sum_{r\in\{0,1\}^p} P_{\hat{X},\Xt\mid R}((\hat{x},\xt)_\swap;r)P_{R}(r)\\
        &=\sum_{r\in\{0,1\}^p} P_{\Xh_m,\Xt_m\mid R}((\xh_m,\xt_m)_{\text{swap}(S\cap m)};r) P_{\Xt_o,\Xh_o\mid R}((\xt_o,\xh_o)_{\text{swap}(S\cap o)};r)P_{R}(r)\\
        &=\sum_{r\in\{0,1\}^p} P_{\Xh_m,\Xt_m\mid R}(\xh_m,\xt_m;r) P_{\Xt_o,\Xh_o\mid R}(\xt_o,\xh_o;r)P_{R}(r)\\
        &=\sum_{r\in\{0,1\}^p} P_{\hat{X},\Xt\mid R}(\hat{x},\xt;r)P_{R}(r)\\
        &=P_{\hat{X},\Xt}(\hat{x},\xt)
        % &=P_{X_o,X_m}(x_o,\hat{x}_m)
\end{align}
\end{subequations}


\ref{proof:uni}b uses the law of total probability, \ref{proof:uni}c follows from univariate sampling i.e. $\Xh_m,\Xt_m\indep \Xh_o, \Xt_o \mid R=r$. \ref{proof:uni}d follows from conditioned on $R=r$, $\Xh_m,\Xt_m$  are \pe and $\Xh_o,\Xt_o$ are \pe.

% $\hat{X}\sim P_{X}$ following Lemma \ref{lem:main1}

% \[(\hat{X},\Xt)_\swap \eqd \hat{X},\Xt\]

\end{proof}

==> chap1/miss/tex/results_hmm.tex <==
% \hm/impute_hmm.pngm}

The experiment results showed that the posterior imputation knockoffs almost always controlled the FDR at the target level ($q=0.1$) irrespective of the amount of missing values and observations (Fig. \ref{fig:heatmap} right). We also observed that increasing the amount of observations ($N$) increased the statistical power while increasing the amount of missing values ($p_0$) decreased it (Fig. \ref{fig:heatmap} left). As a matter fact as $p_0$ got closer to 0.45 the power reduced to $0$ irrespective of $N$. 

% As the amount of missing data and the number of observations both have contradicting affects on the statistical power, a natural question arises as whether the power can be kept constant. As an example, 2000 samples with $15\%$ missing values have power comparable to 1125 samples. For that purpose we have drawn the constant power contours (Fig. \ref{fig:contour}). We have observed that the constant power contours are not linear and tolerating a increase in missing value amount gets more challenging. For example, when $N=1000$ to tolerate an increase in $p_0$ by one unit, additional two units of samples are required. However, when $N=1625$ to compensate a one unit increase in $p_0$ three units of samples are required.  

We observed that Algorithm \ref{alg:sesia} also controlled the FDR control (Appendix Fig. \ref{fig:heatmap2} right). In terms of power it's difficult to distinguish the Algorithm \ref{alg:sesia} and Algorithm \ref{alg:main} (Appendix Fig. \ref{fig:contour}). That suggests the computational advantages of Algorithm \ref{alg:sesia} do not have a shortcoming in performance.

% We have also observed that the slops of the constant power contours vary. For example: to tolerate an increase in $p_0$ by 1 unit, additional 2 units of samples when $N=1000$, while when $N=1625$, 3 units of samples are required.

%https://www.wolframalpha.com/input/?i=y%2F%281-y%29%3Dx

% For $p_0$ values higher than $0.45$ like power, FDR is also close to 0. For $p_0$ values lower than $0.45$, FDR is around $q=0.1$. 

% \textbf{Results }Power and FDR values corresponding to the searched parameters are displayed in Fig. \ref{fig:heatmap}. When $N$ is largest and $p_0$ is lowest, the highest power is achieved (right bottom of the figure). As $p_0$ gets closer to 0.45 the power reduces to $0$ irrespective of $N$. Decreasing the $p_0$ (moving towards the top) tends to reduce power for all the $N$ values and increasing $N$ (moving towards the right) tends to increase the power. Average FDR is less than $q=0.1$ most of the time irrespective of $p_0$ and $N$. For $p_0$ values higher than $0.45$ like power, FDR is also close to 0. For $p_0$ values lower than $0.45$, FDR is around $q=0.1$. 



% In the HMM An interesting question can be understanding whether the relationship is linear across the grid or not.
% These simulation supports the theoretical results that FDR control is possible under missing data. Moreover, it shows reasonable power can be obtained at least under the low correlation setting.


% One would prefer the FDR to be closer 


% supports the theory which suggest 


\begin{figure}[!h]
    \centering
    \includegraphics[width=1.\linewidth]{img/hmm/new/post_hmm_crop.png}
    % {img/hmm/impute_hmm.png}
    % {img/Picture2_fill.png}
    \caption{Heatmap of power on the left, FDR on right. The posterior imputation + Sesia HMM Knockoffs is used (Algorithm \ref{alg:main}). On the left darker red (blue) indicates higher (lower) power. On the right values above $q=0.1$ are red and below are blue.}
    \label{fig:heatmap}
\end{figure}


% Contour plots (Fig: \ref{fig:contour})



% Therefore visual inspection suggests slope decreases as $N$ incr.

% Upon visual inspection of the figure \ref{fig:contour}, different constant power lines have similar slopes and 
% similar slopes after $N=1000$. 

% The contour plots are somewhat vague as more points on the searched grid are needed.

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=1.\linewidth]{img/hmm/left_impute_contr.png}
%     \caption{Contour plots of power. Each cross is a searched pair. Interpolation is used to to draw constant power lines. Left: the posterior imputation + Sesia HMM Knockoffs (Algorithm \ref{alg:main}), Right is the Modified Sesia HMM Knockoffs (Algorithm \ref{alg:sesia})}
%     \label{fig:contour}
% \end{figure}



==> chap1/miss/tex/results_mvn.tex <==
\paragraph{Results}

Same experiment parameters $p=1000$, $a=0.32$, $\mid S\mid =60$ are used. We have varied $p_0=\{0,0.1,\dots,0.4\}$, and $\rho=\{0,0.1,\dots,0.8\}$ but kept $N=1500$. Due to computational limitations experiments are repeated 31 times.  

We can observe that as correlation increases the x axis power decreases similarly as $p_0$ increases power decrease. The FDR is controlled.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.\linewidth]{img/Picture2_rho.png}
    \caption{Heatmap of power on the left, FDR on right. X axis is $\rho$ and y axis is $p_0$. On the left darker red (blue) indicates higher (lower) power. On the right values above $q=0.1$ are red and below are blue.}
    \label{fig:heatmap}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.\linewidth]{img/Picture1_rho.png}
    \caption{Contour plots. Each cross is a searched pair. X axis is $\rho$ and y axis is $p_0$. Power on the left, FDR on right. Interpolation is used to to draw constant power (or FDR) lines.}
    \label{fig:contour}
\end{figure}

==> chap1/miss/tex/results_mvn_p700.tex <==
% \paragraph{Results}

% and average FDR is generally controlled at the target $q=0.1$ (Fig \ref{fig:mvn3})

After conducting the experiments, we have observed that the average FDR is generally controlled at the target $q=0.1$ regardless of number of missing values, and the correlation amount (Fig \ref{fig:mvn_double}). We also noticed that as $\rho$ increased the average power consistently decreased (Fig \ref{fig:mvn_double}).increasing the number of missing values ($p_0$) decreased the power (Fig \ref{fig:mvn_double}). 

% The simulations also suggest that the average FDR is generally controlled at the target $q=0.1$ regardless of the missing value pattern (Fig \ref{fig:mvn3}).
 
%  When $\rho=0.7$ and $\rho=0.8$, the as $p_0$ increased power increased in the univariate imputation but decreased in the posterior imputation.

% To an extend when $p_0=0.4$ it decreased almost to zero. 

We have compared the statistical power of posterior and univariate imputation knockoffs (Fig \ref{fig:mvn2}). The posterior imputation has an advantage (Fig \ref{fig:mvn2} right). That advantage is less visible for lower $\rho$ values and one reason is the MSE of the posterior imputations depends on $\rho$. 
% especially when $\rho$ is around 0.5.
As $\rho$ increases, the conditional variance of the missing values decreases. That doesn't change the MSE of the univariate imputation but translates into a to lower MSE for the posterior imputation. As $\rho$ increases further the power difference starts to shrink again, possibly because of resulting intrinsically difficulty problem.
% the power for both methods becomes closer to the lower bound 0.

% . Univariate imputation, Despite having higher MSE statist

% The power difference between the univariate and the posterior imputation methods depends on both $\rho$ and $p_0$ (Fig \ref{fig:mvn2}). In the first and the third settings when $\rho<0.5$ the power difference is less than $0.1$ but when $\rho\geq0.5$ the advantage of posterior imputation becomes more apparent. However, as $p_0$ reaches $0.4$ the gap decreases again. The second setting is different. When $\rho\geq0.6$, the power gap starts to increase but it increases in favor of univariate imputation. When $\rho\geq0.7$ the gap is more visible when $p_0\geq0.3$.

% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[width=.8\linewidth]{img/mvn/contr.png}
%     \caption{Constant power contours of the posterior imputation knockoffs. The missing value positions are restricted to true features on the \emph{left}, to null features on the \emph{middle}, and are not restricted on the \emph{right}. Each cross is a searched pair. X axis is $\rho$ and y axis is $p_0$. Interpolation is used to to draw the constant power lines.}
%     \label{fig:mvn1}
% \end{figure*}
\begin{figure*}[]%!htb
    \centering
    \includegraphics[width=0.4\linewidth]{diff_3.png}
    \caption{Heatmap of power difference between posterior (Algorithm \ref{alg:main}) and univariate (Algorithm \ref{alg:uni}) imputation methods. Darker red (blue) indicates posterior imputation has a higher (lower) power. X axis is $\rho$ and y axis is $p_0$. One sided Mann-Whitney U rank test is applied to get the uncorrected p-values and statistical significance levels are denoted by *:0.05, **:0.01, ***:0.001, ****:0.0001. No stars indicates not significant.}
    \label{fig:mvn2}
\end{figure*}


% \begin{figure}
%     \centering
%     \includegraphics[width=.9\linewidth]{3.png}
%     \caption{Heatmap of power on the left, FDR on right. The posterior imputation + MVN Knockoffs is used. Y axis changes the missing value amount ($p_0$) and x axis the correlation amount ($\rho$). FDR is generally controlled $<0.1$.
%     }
%     % Increasing the amount of correlation and missing values
%     % On the left darker red (blue) indicates higher (lower) power. On the right values above $q=0.1$ are red and below are blue.}
%     \label{fig:my_label}
% \end{figure}

% Another comparison we made was between the three readily available imputation methods 
% that do not guarantee FDR control under the knockoffs framework 
% and the methods we introduced. Those three methods are K-nearest neighbour (KNN) imputation \cite{troyanskayaMissingValueEstimation2001}, SoftImpute \cite{mazumderSpectralRegularizationAlgorithms2010}, and sample mean imputation. We have used scikit-learn for KNN imputation which fills the missing values of a row by the average of the closest (in Euclidean geometry) K rows \cite{scikit-learn} and sample mean imputation which imputes the missing values with the column's sample mean. SoftImpute, implemented in \cite{rubinsteynIskandrFancyimpute2021} fancyimpute package, is an SVD decomposition-based iterative matrix completion algorithm. We have used the third experimental setting i.e. no restriction on the position of missing values.

% We have observed that the off-the-shelf methods had generally higher power than the posterior and univariate methods (Figure \ref{fig:mvn4} left). Despite the three off-the-shelf methods violate the independence assumption of the rows and the equality between the distributions $P_{\hat{X}}$ and $P_X$, we observed that they control the FDR (Figure \ref{fig:mvn4} right). That can possibly be due to $P_{\hat{X}}$ being ``close'' to $P_X$ in our experiments, and the robustness of the knockoffs framework \cite{barberRobustInferenceKnockoffs2019}. More experimentation with different predictor and target distributions can help to understand the conditions of FDR control with off-the-shelf imputation methods.

% Before generalizing the empirical advantages of the off-the-shelf methods further studies with varying explanatory and response distributions should be conducted.

% the-off-the shelf imputation algorithms doesn't guarantee the closeness of the probability distributions, to ad empirical experiments with different probability distributions are require
% That can be expected under the assumption stribution errors 



% \begin{figure}[!htb]
% % [!htb]
%     \centering
%     \includegraphics[width=1\linewidth]{img/mvn/new/mvn_fdr.png}
%     \caption{Heatmap of FDR of the posterior imputation method (Algorithm \ref{alg:main}). The missing value positions are restricted to true features on the \emph{top left}, to null features on the \emph{top right}, and are not restricted on the \emph{bottom}. X axis is $\rho$ and y axis is $p_0$. Values above $q=0.1$ are red and below are blue.}
%     \label{fig:mvn3}
% \end{figure}

% Among the different imputation methods, when features are less correlated ($\rho\leq0.5$), the mean imputation method has the highest power. When $\rho>0.5$ and $p_0$ $\leq0.3$, SoftSVD has slightly higher power than the rest. Average FDR is also generally under the target $q=0.1$ for both the ones with and without a theoretical guarantee. When the missing amount is the highest ($p_0=0.4$), the off-the-shelf methods slightly overshoot when $\rho=0.5$. 

% \begin{figure*}[]%!htb
%     \centering
%     \includegraphics[width=1.\linewidth]{img/mvn/impute_fig_sub.png}
%     \caption{Comparison of different imputation methods. Left column is power vs $\rho$ and right column is FDR vs $\rho$. Rows corresponds to different amounts of missing data. From top to bottom $p_0$ takes the values $\{0.2, 0.4\}$. The corresponding color and line style of the imputation methods are denoted in the legend. The full figure is given in Appendix Figure \ref{app:fig:mvn4}.}
%     \label{fig:mvn4}
% \end{figure*}



% A more detailed simulation where $p_0$ should show that below a certain point there isn't a difference.


% In this setting because the missing values do not occur in the true covariates, increasing their amount has less effect on the power.


% In the second experimental setting, the univariate imputation tends to have higher power than the posterior imputation.

% imputed nulls and true covariates become uncorrelated when univariate imputation is used but correlated when posterior imputation is used. 

% One can also expect because the missing values are all in null the amount of $p_0$


 

% for the additional correlation introduced among the missing nulls and observed true variables. 


% One can also state that lower MSE on the true covariates compensates for the additional correlation introduced among the missing nulls and observed true variables. 



% Although, the correlation among the missed and observed variables increase with posterior method 

% The constrast between the second and third experimental settings indicate that 


% it's more important 

% the missing values are restricted to null-variables increasing the correlation between 
% suggesting 

% comes with the cost of additional correlation among

% The MSE of the imputations of the true covariates is what matters difference as the second experimental setting demonstrates only effects on 

% missing values 

% $p_0$ has two different effects on the power. When the $\rho\geq0.6$ a



% Also, it interesting 

% And, it seems that the Another reason can be the MSE in the imputed nulls is not as crucial as the imputed true covariates.



% the correlation between true covariates and imputed nulls is higher with the posterior imputation. 


%The difference becomes more observable as $\rho$ increases where when  $\rho=0.8$ the difference can be up to 0.21. 

% lower MSE in the nulls does not translate to a higher power which can 


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.\linewidth]{example-image-a}
%     \caption{Contour plots. Each cross is a searched pair. X axis is $\rho$ and y axis is $p_0$. Power on the left, FDR on right. Interpolation is used to to draw constant power (or FDR) lines.}
%     \label{fig:contour}
% \end{figure}

==> chap1/miss/tex/theory_err.tex <==
% \subsection{Mean Squared Errors (MSEs) of Two Imputation Methods}
\subsection{Comparing the Imputation Performance}
% For simplicity, $\E[Y]=0$.

% \subsubsection{MSE for first imputation}

Maintaining the \pety is required for controlling the FDR but in practise one is also interested in maximizing the statistical power. As we have shown both Alg. \ref{alg:main} and Appendix Alg. \ref{alg:uni} maintains the \pety but they're not equal in terms of the imputation quality.

A standard approach for measuring the imputation quality is the Mean Squared Error (MSE). It's well known fact that optimal MSE estimator which is given by
the mean of the posterior. But the method we use, posterior sampling, is not optimal as it takes a sample from the posterior. The next proposition illustrates that:
% We like to underline the distin

% \subsubsection{Comments}
\begin{prop}\label{thm:err}
Let $Y$ denote a R.V, $X$ denote a random vector. Given the following three estimators $Y'\sim P_Y(\cdot), \ Y''\sim P_{Y\mid X}(\cdot;X),\ Y'''=\E[Y\mid X]$, their MSEs has to satisfy $ \E[(Y-Y''')^2]\leq \E[(Y-Y'')^2]\leq \E[(Y-Y')^2]$.
\end{prop}
Proof is in \ref{app:err}. The proposition states that Algorithm \ref{alg:main} although not optimal is expected have lower (or equal) imputation error then univariate sampling (Appendix Algorithm \ref{alg:uni}). The reason we're not using the optimal estimator is it's deterministic and does not preserve the distribution. In certain scenarious (ex: markov chains) using deterministic imputation can require the knockoffs of the missing values to be exactly equal to their originals i.e. $\Xt_m=\Xh_m$ that would decrease the statistical power.

% These results suggests that assuming lower imputation error leads to a better performance, posterior imputation should be preferred over the univariate. However, our goal is not to have the optimal MSE estimator which is given by
% $Y''=\E[Y\mid X]$ because in general $Y''\neqd Y$ and one cannot directly use the existing knockoff samplers.

==> chap1/miss/tex/theory_post2.tex <==
\section{Extending the Model-x Framework to Missing Data}
% \input{tex/proof_mar}


% In this work, we will introduce different ways for dealing with missing data under the knockoffs framework. Throughout this work, we denote $X=(X_1,\dots,X_p)^T$ as the exploratory R.Vs and $R=(R_1,\dots,R_p)^T$ denote the missing value indicator R.Vs. $R_i$ takes values in $\{0,1\}$ and $R_i=1$ denotes $X_i$ is missing. Let $m=\{i:R_i=1\}$ and $o=\{1,\dots,p\}\setminus m$ denote the sets of missing and observed values. Given a set $S\subseteq\{1,\dots,p\}$, $X_S=\{X_i:i\in S\}$ denotes the R.Vs indexed by set S.

Just as valid p-values requires the assumptions of the statistical tests to be justified, the assumptions of the model-x knockoffs needs to be justified to control the FDR. As illustrated in Eq.\ref{eq:back}, imputation of missing data can add further complications. Instead, we will show that it's possible to do imputation without making additional assumptions. The idea is because the distribution of $X$ needs to be known for model-x knockoffs, there is no reason for not using $P_X$ for imputation as well.
% Model-x framework is based on the idea that we have an accurate model for  also determines the optimal imputation algorithm.

\subsection{Knockoffs for Posterior Sampled Missing Values}
Our first solution referred to as posterior sampled imputation aims to use keep the imputed vectors distribution intact. That is practically very useful because a knockoff sampler $P_{\Xt \mid X}$ of $P_X$ which is already implemented can be applied directly to the imputed matrix. The following Lemma \ref{lem:mar} illustrates the idea.

% We start by introducing the posterior sampled missing value knockoffs method which allows reusing the existing knockoff samplers under MAR and MCAR. 

\begin{lem}\label{lem:mar}
Let $\Xh=(\Xh_1,\dots,\Xh_p)^T$ denote the imputed vector where $\Xh_o=X_o$. If $\hat{X}_m\sim P_{X_m\mid X_o,R}(\cdot;X_o,R)$ and then $P_X=P_{\Xh}$.
\end{lem}
The proof simply uses Eq. \ref{eq:back} and replaces $Q$ with $P_{X_m\mid X_o,R}(\cdot;X_o,R)$. It's unrealistic in practise to assume the joint distribution of the exploratory variables and the missing data pattern i.e. $P_{X,R}$ to be known. Therefore, we focus our attention on two missing data configurations namely configurations Missing Completely At Random (MCAR) and Missing At Random (MAR) \citep{littleStatisticalAnalysisMissing2002a}. MCAR holds if $X \indep R$ holds and MAR holds if $X_m \indep R \mid X_o$ holds for any $X_m,X_o$ \cite{littleStatisticalAnalysisMissing2002a,mohanGraphicalModelsInference2017}.

\begin{cor}\label{cor:mar}
Under MAR or MNAR, if $\hat{X}_m\sim P_{X_m\mid X_o}(\cdot;X_o)$ then $P_X=P_{\Xh}$.
\end{cor}
The proof simply follows directly from the conditional independence assumptions of MAR and MNAR. Corollary \ref{cor:mar} is more realistic as it only requires the distribution $P_X$ which we already assumed to be known. We formalize our idea of posterior sampled imputation and reusing a knockoff sampler in the following step.



% The idea behind the first algorithm is simple, 
% The knockoffs framework assumes that the input distribution $P_X$ is known or known to a certain accuracy. That information can be used for imputation in such a way that the FDR control is maintained. The idea is if we can sample $\hat{X}_m$ from the posterior distribution $P_{X_m\mid X_o}$ than the joint distribution of $\hat{X}$ will remain unchanged. More importantly existing knockoff samplers can be used with the same FDR guarantees. 
\vspace{0.5cm}
\begin{definition} Following \cite{barberRobustInferenceKnockoffs2019} a conditional distribution $P_{\Xt\mid X}$ is pairwise exchangeable with respect to a probability distribution $Q_{X}$ if given
$X\sim Q_X(\cdot)$ and $\Xt \sim P_{\Xt\mid X}(\cdot;X)$, $X$ and $\Xt$ are pairwise exchangeable.

\end{definition}


\begin{thm}\label{thm:main}
Let $\Xh=(\Xh_1,\dots,\Xh_p)^T$ denote the imputed vector where $\hat{X}_m\sim P_{X_m\mid X_o}(\cdot;X_o)$ and $\Xh_o=X_o$. We assume the distribution $P_{X,R}$ satisfies MCAR or MAR. If $\Xt \sim P_{\Xt\mid X}(\cdot;\hat{X})$ and $P_{\Xt\mid X}$ is pairwise exchangeable with respect to $P_X$, then $\hat{X}$ and $\Xt$ are pairwise exchangeable.
\end{thm}

% \paragraph{Proof}
\begin{proof}[Proof of Theorem \ref{thm:main}]
% Let $x=(x_o,x_m)^T$,

% \begin{equation}
%     \begin{split}
%         P_{\hat{X}}(x)&=P_{X_o,\hat{X}_m}(x_o,\hat{x}_m)\\
%         &=P_{\hat{X}_m\mid X_o}(\hat{x}_m;x_o)P_{X_o}(x_o)\\
%         &=P_{X_m\mid X_o}(\hat{x}_m;x_o)P_{X_o}(x_o)\\
%         &=P_{X}(x)
%         % &=P_{X_o,X_m}(x_o,\hat{x}_m)
%     \end{split}
% \end{equation}
Following from Corrollary \ref{cor:mar}, $P_{\Xh}(x)=P_X(x)$ holds for all $x$ under MAR or MCAR. Then $P_{\Xt\mid X}$ is pairwise exchangeable with respect to $P_{\hat{X}}$ and by the definition of a pairwise exchangeable distribution $\hat{X}$ and $\Xt$ are pairwise exchangeable.
% $\hat{X}\sim P_{X}$ following Lemma \ref{lem:main1}

% \[(\hat{X},\Xt)_\swap \eqd \hat{X},\Xt\]

\end{proof}
Given that we proved our approach results in \pe pairs, in Algorithm \ref{alg:main} we illustrate how it can be applied to N i.i.d. observations $\{x^{(i)}_{o^{i}}\}_{i=1}^N$ with varying missing values indices $\{m^{i},o^{i}\}_{i=1}^N$. The only additional step introduced in Algorithm \ref{alg:main} is the sampling the missing values from the posterior.
% Because of the i.i.d. assumption the resulting imputed matrix and knockoffs matrix will be pairwise exchangeable as well. 


% given N observations $\{x^{(i)}_{o^{i}}\}_{i=1}^N$ 

% \begin{algorithm}[H]
\begin{algorithm}[]
\caption{Posterior sampled missing value knockoffs}\label{alg:main}
%   \textbf{Input:}  $\{x^{(i)}_{o^{i}}\}_{i=1}^N, \{m^{i},o^{i}\}_{i=1}^N, P_{\Xt\mid X}, P_X$
\begin{algorithmic}
\STATE {\bfseries Input:} $\{x^{(i)}_{o^{i}}\}_{i=1}^N, \{m^{i},o^{i}\}_{i=1}^N, P_{\Xt\mid X}, P_X$
    \FOR{\texttt{$i=1,\dots,N$}}
        \STATE $m\leftarrow m^i$
        \STATE $o\leftarrow o^i$
        \STATE $\hat{x}_{m}\sim P_{X_{m}\mid X_{o}}(\cdot;x^{(i)}_{o})$ \hfill\COMMENT{Posterior Imputation}
        \STATE  $\hat{x}^{(i)}\leftarrow(x^{(i)}_{o},\hat{x}_{m})$
        \STATE$\xt^{(i)} \sim P_{\Xt\mid X}(\cdot;\hat{x}^{(i)}) $\hfill\COMMENT{Knockoff Sampling}
    \ENDFOR
\STATE {\bfseries Output:} $\{\hat{x}^{(i)},\xt^{(i)}\}_{i=1}^N$
\end{algorithmic}
\end{algorithm}


==> chap1/miss/tex/theory_rndm.tex <==
% introduce a simple and general method for sampling knockoffs 
\subsection{Knockoffs for Univariate Sampled Missing Values}

% We also provide a simpler algorithm which doesn't require sampling from the posterior distribution. 
If we have an valid knockoff generator for the observed variables $P_{X_o}$ but sampling from the posterior is challenging then we can use the below Algorithm \ref{alg:uni}. One can show that the Algorithm \ref{alg:uni} is a valid knockoff generator because of the univariate sampling of the missing values. 

% \begin{algorithm}[H]\label{alg:uni}
% \caption{Univariate sampled missing value knockoffs}
%     Input: $x_o, P_X, \mathcal{A'}$\\
%         % \SetAlgoLined
%             $\xt_o \sim \mathcal{A'}(x_o,P_{X_o}) $\\
%              \For {i= 1,...,$|o|$}{
%             $\hat{x}_{m_i}\sim P_{X_{m_i}}(\cdot)$ \\
%             $\xt_{m_i}\sim P_{X_{m_i}}(\cdot)$ \\
%             }
%             $x_c\leftarrow(x_o,\hat{x}_m)$\\
%     Output: $x_c,\xt$
% \end{algorithm}


\begin{algorithm}[H]
\caption{Univariate sampled missing value knockoffs}\label{alg:uni}
 \textbf{Input:} $x_o, P_X, \mathcal{A'}, m, o$
\begin{algorithmic}
\State $\xt_o \sim \mathcal{A'}(x_o,P_{X_o}) $
 \For {i= 1,...,$|m|$}
    \State $\hat{x}_{m_i}\sim P_{X_{m_i}}(\cdot)$ 
    \State $\xt_{m_i}\sim P_{X_{m_i}}(\cdot)$ 
\EndFor
    \State $x_c\leftarrow(x_o,\hat{x}_m)$
\end{algorithmic}
\textbf{Output:} $x_c,\xt$ 
\end{algorithm}



% Furthermore, if $P_{X_{m_i}}$ is also not strictrily required any univariate distribution

==> chap1/miss/tex/theory_uni.tex <==
% introduce a simple and general method for sampling knockoffs 
\subsection{Knockoffs for Univariate Sampled Missing Values}

% We also provide a simpler algorithm which doesn't require sampling from the posterior distribution. 
In scenarios where sampling from the posterior is challenging but knockoffs for the observed R.Vs $X_o$ can be sampled, an alternative method can be using univariate imputation. First the knockoffs for the observed variables $\Xt_o$ will be sampled then the missing values of the originals $\hat{X}_m$ and the knockoffs $\Xt_m$ will be imputed independent from $X_o,\Xt_o$. 

% If one can sample knockoffs for the observed variables $P_{X_o}$ and cannot sample from the posterior distribution, then an alternative approach can be followed. First, we sample the knockoffs for the observed variables and

% use the below Algorithm \ref{alg:uni}. 

\begin{thm}\label{thm:uni}

Let $\Xh=(\Xh_1,\dots,\Xh_p)^T$ denote the imputed vector where $\Xh_o=X_o$ and $\hat{X}_{m_j}\sim P_{X_{m_j}} \ j=1,\dots, |m|$. We assume $P_{X,R}$ satisfies MAR or MCAR. If $\Xt_o \sim P_{\Xt_o\mid X_o}(\cdot;\hat{X_o})$, $P_{\Xt_o\mid X_o}$ is pairwise exchangeable with respect to $P_{X_o}$, and $\Xt_{m_j}\sim P_{X_{m_j}} \ j=1,\dots, |m|$ then $\hat{X}$ and $\Xt$ are pairwise exchangeable.
\end{thm}

The proof is in Appendix \ref{app:uni}. The intuition of the proof is because of the independence between the imputed variables and the observations i.e. $\Xh_m \indep \Xh_o$, \pety needs only to be satisfied within missing variables and observed variables separately. Notice that in the posterior sampled imputation our goal is to preserve the distribution of $X$ but in the univariate our goal is the opposite. We sacrifice the dependence between $X_{m}$ and $X_o$ to make the \pe condition easier to satisfy. 

In Appendix Algorithm \ref{alg:uni}, we have described how this can be applied to N i.i.d. observations. Notice that for each different set of observed variables $o^i$ a different knockoff sampler $P_{\Xt_{o^i}\mid X_{o^i}}$ is required. That is computationally a disadvantage compared to Algorithm \ref{alg:main}. But Appendix Algorithm \ref{alg:uni} has a computationally easier imputation step as it samples from the univariate distribution instead of the posterior.

% One can show that the Algorithm \ref{alg:uni} is a valid knockoff generator because of the univariate sampling of the missing values. 

% \begin{algorithm}[H]\label{alg:uni}
% \caption{Univariate sampled missing value knockoffs}
%     Input: $x_o, P_X, \mathcal{A'}$\\
%         % \SetAlgoLined
%             $\xt_o \sim \mathcal{A'}(x_o,P_{X_o}) $\\
%              \For {i= 1,...,$|o|$}{
%             $\hat{x}_{m_i}\sim P_{X_{m_i}}(\cdot)$ \\
%             $\xt_{m_i}\sim P_{X_{m_i}}(\cdot)$ \\
%             }
%             $x_c\leftarrow(x_o,\hat{x}_m)$\\
%     Output: $x_c,\xt$
% \end{algorithm}






% Furthermore, if $P_{X_{m_i}}$ is also not strictrily required any univariate distribution
